RADIUS: Risk-Aware, Real-Time, Reachability-Based Motion Planning

Deterministic methods for motion planning guarantee safety amidst uncertainty in obstacle locations by trying to restrict the robot from operating in any possible location that an obstacle could be in. Unfortunately, this can result in overly conservative behavior. Chance-constrained optimization can be applied to improve the performance of motion planning algorithms by allowing for a user-specified amount of bounded constraint violation. However, state-of-the-art methods rely either on moment-based inequalities, which can be overly conservative, or make it difficult to satisfy assumptions about the class of probability distributions used to model uncertainty. To address these challenges, this work proposes a real-time, risk-aware reachability-based motion planning framework called RADIUS. The method first generates a reachable set of parameterized trajectories for the robot offline. At run time, RADIUS computes a closed-form over-approximation of the risk of a collision with an obstacle. This is done without restricting the probability distribution used to model uncertainty to a simple class (e.g., Gaussian). Then, RADIUS performs real-time optimization to construct a trajectory that can be followed by the robot in a manner that is certified to have a risk of collision that is less than or equal to a user-specified threshold. The proposed algorithm is compared to several state-of-the-art chance-constrained and deterministic methods in simulation, and is shown to consistently outperform them in a variety of driving scenarios. A demonstration of the proposed framework on hardware is also provided.

==> sections_long/01_introduction.tex <==
\section{Introduction}\label{sec:intro}

For robots to safely operate in unstructured environments, they must be able to sense their environments and develop plans to dynamically react to changes while avoiding obstacles. 
% Safe navigation through these uncertain environments in the presence of dynamic obstacles is a critical challenge. 
Unfortunately, it is challenging to accurately and precisely estimate and predict an obstacle's movement. 
For robots to operate robustly, the uncertainty within these estimations and predictions must be accounted for while generating motion plans.
Various approaches to account for this uncertainty have been proposed in the literature, but these methods either (1) have difficulty being utilized in real-time, (2) make strong assumptions on the class of probability distributions used to model the uncertainty, or (3) generate motion plans that are overly conservative and thereby restrict motion.
This paper develops an algorithm called \textbf{\riskmethodname{}} (introduced in Fig. \ref{fig:RiskRTD-intro}) for \textbf{real-time, risk-aware motion planning} while addressing each of the aforementioned challenges.

We begin by summarizing related algorithms for safe motion planning under uncertainty.
Approaches to address this problem can be broadly categorized as deterministic or stochastic. 
The deterministic approaches often assume some bounded level of uncertainty and solve for motion plans that are robust to this bounded uncertainty. 
Reachability-based methods \cite{RTD}\cite{REFINE} for instance, over-approximate the uncertain regions using level sets of polynomials or polytopes and plan paths that do not intersect with these regions. 
As we illustrate in this paper, such methods may be overly conservative as they must over-approximate the uncertain region to include events that may have an exceedingly small probability of occurring to ensure safety.

\begin{figure}[t]
    \centering
    % \includegraphics[width=1\columnwidth]{figures/Overview_Figure_Draft_1.pdf}
    % \includegraphics[trim={0cm, 10.5cm, 16.4cm, 0cm},clip,width=1\columnwidth]{figures/big_pic.pdf}
    \includegraphics[trim={0cm, 10.5cm, 16.4cm, 0cm},clip,width=1\columnwidth]{figures/big_pic_v3.pdf}
    \caption{An illustration of the motion planning framework Risk-RTD that is developed in this paper. 
    Risk-RTD first performs offline reachability analysis using a closed-loop full-order vehicle dynamics to construct a control-parameterized, zonotope reachable set (shown as dark gray boxes) that over-approximates all possible behaviors of the ego vehicle over the planning horizon. 
    % During online planning, Risk-RTD first determines the appropriate level of risk ($\epsilon{}$) based on the likelihood of serious injury should a crash occur at the current velocity. 
    During online planning, given some user-defined level of risk of collision ($\epsilon{}$) for the motion plan, \riskmethodname{} constructs a trajectory by solving an optimization problem that selects subsets of pre-computed zonotope reachable sets that are certified to have a less than $\epsilon$ chance of colliding with any obstacles. 
    In this figure, the moving obstacles shown in white and the 3-$\sigma$ regions of the corresponding probability distributions for the obstacle locations are shown as the purple and blue ellipses where the probability density from low to high is illustrated from blue to purple.
    The subsets of the dark gray zonotope reachable sets corresponding to the trajectory parameter shown in green ensures a collision-free path that is guaranteed to have a less than $\epsilon$ chance of colliding with all obstacles, while the two trajectory parameters and their corresponding reachable sets shown orange may have a greater than $\epsilon{}$ chance of collision with the moving obstacles.}
    \label{fig:RiskRTD-intro}
    \vspace*{-0.5cm}
\end{figure}

Stochastic methods incorporate probabilistic information about the environment to reduce the level of conservativeness of their motion plans. 
Many of these methods leverage chance constraints that allow for some user-specified amount of constraint violation. 
For instance, sampling-based algorithms for chance constrained motion planning apply numerical integration techniques to compute the probability of collision \cite{janson2018monte,asmussen2007stochastic}. 
In this context the chance constraint is expressed as an indicator function on the set of variables that violate the collision constraint. 
Random samples are drawn from the uncertain region and the weighted sum of these samples is taken to approximate the integral. 
These methods are simple to implement, but can be computationally expensive \stkout{and have slow convergence rate} \new{as they require large numbers of samples to converge to a good estimate of the probability of collision.}
\Ram{what does slow convergence rate mean?}. \challen{Addressed.}
Moreover, they are difficult to utilize in gradient-based optimization algorithms due to the non-smooth nature of the indicator function used as the integrand. 
To address these limitations, moment-based methods upper bound the probability of collision using the moments of the probability distribution  \cite{wang2020,wang2fast,cantelli1929sui}. 
Recent works leverage MPC and SOS programming in conjunction with these moment-based upper bounds to perform motion planning. 
Unfortunately, these methods can be conservative as the bound must \stkout{exist} \new{be valid} \Ram{I don't think exist is the right word here. The bound always exists.} \challen{Addressed} for all distributions with the given moments.
Coherent risk measures like conditional value-at-risk (CVaR) and Entropic value-at-risk (EVaR) have been used to regulate safety by limiting the expectation of the distance to the safe region using a worst-case quantile representation of a distribution \cite{hakobyanCVAR}\Ram{cite some cvar papers...}. \challen{Addressed.}
However, CVaR constraints are difficult to construct directly due to the computationally expensive multi-dimensional integration that is required.
As a result, they are often approximated using sampling methods \new{which as mentioned earlier can be computationally expensive.} \Ram{what is the problem with approximating that style of approximation?}. \challen{Addressed.}
Moreover, developing real-time algorithms to solve optimization problems with CVaR constraints is challenging because they typically require performing mixed-integer programming \cite{hakobyanCVAR} \Ram{there are people who do mixed integer linear programming in real-time...so just because you are mixed integer doesn't make you bad.}. 
Branch-and-bound methods like the Chance Constrained Parallel Bernstein Algorithm (CCPBA) use reachability-based methods in conjunction with a branch-and-bound style algorithm to compute tight bounds for the probability of collision \cite{SeanFast}. 
However, to compute these probabilities they assume an \textit{a priori}, closed-form, formula for the cumulative distribution function that can be evaluated during online optimization. 
Such a representation for the cumulative distribution function is typically not available except for the simplest classes of probability distributions (\emph{e.g.}, Gaussian).


% Another challenge while using chance constrained programming is identifying how select the level of constraint violation. 
% Most stochastic planning methods select this parameter arbitrarily, and evaluate the agent performance at various risk thresholds \cite{lyons_chance,wang2020,SeanFast}.
% For long-term autonomy in the real-world, agents must be able to determine how to select this violation as a function of their surrounding.
% As such these agents should be able to vary their risk thresholds in an appropriate manner to balance conservativeness and safety.

\challen{Contribution order needs to be updated once things are finalized}
\Ram{also need to give an outline of how the paper is organized.}
This paper makes the following contributions.
% First, it presents a framework for systematically varying the level of safety and conservativeness of a the motion plans based on the risk of serious injury to the passenger (Section \ref{sec:risk threshold}).
First, it provides a novel closed-form over-approximation of the probability of a collision with an obstacle given an arbitrary probability distribution from the exponential family (Section \ref{subsec:chance constraint}).
Second, it describes an analytical derivative of the probability over-approximation with respect to the control parameters (Section \ref{subsec:gradient})
Third, this paper presents a parallelized method to perform real-time, risk-aware motion planning by select trajectories that guarantee safety up to the given risk threshold (Section \ref{subsec:cuda}).
Lastly, this paper describes a demonstration of \riskmethodname{} in simulation and on hardware, plus a comparison to \methodname{}, CCPBA, and Cantelli MPC in on a number of dense highway scenarios. (Section \ref{sec:experiments}).

% For brevity, we provide self-collision constraints and all proofs in our supplementary material.
% \pat{make sure we link to supplement before submitting}

% \pat{Do we want to come out and say here that we're only dealing with static obstacles but the extension to dynamic obstacles is straightforward?}
% \shrey{done above}

% \subsection{Notation}
% The $n$-dimensional real numbers are $\R^n$, natural numbers are $\N$, the unit circle is $\s^1$, and the set of $3\times 3$ rotation matrices is $\SO(3)$.
% Vectors are either $[x_1,\cdots,x_n]^\top$ or $(x_1,\cdots,x_n)$ depending on if the size/shape is relevant.
% Let $U, V \subset \R^n$.
% For a point $p \in U$, $\{p\} \subset U$ is the set containing $p$.
% The power set of $U$ is $\P(U)$.
% The Minkowski sum is $U \oplus V = \{u + v~|~u \in U,\ v \in V\}$.
% For a matrix $A \in \R^{n\times n}$, $AU = \{Au~|~u \in U\}$.
% For matrices, $\prod$ performs right multiplication with increasing index (e.g., $\prod_{i=1}^3 A_i = A_1A_2A_3$).
% Greek lowercase letters in angle brackets are indeterminate variables (e.g., $\sym{\sg}$).
% Superscripts on points index elements of a set.
% Subscripts are joint indices or contextual information.


==> sections_long/02_03_Notation_and_Preliminaries.tex <==
\section{Notation}
\label{sec: notation}

% and the notion of safety that is enforced throughout the remainder of this manuscript.

% \subsection{Notation}
% \label{subsec: notation}


% Sets and subspaces are typeset using calligraphic font.
% Superscripts are used for descriptive words \Ram{what does a descriptive word mean?}.
% Subscripts are used to follow conventional notations in the literature. 
% Subscripts are primarily used as an index or to describe an particular coordinate of a vector.

% \subsection{Notations}
% This section defines the set representations and notation that are used throughout the remainder of this manuscript.

This section formalizes notation used throughout the paper.
Sets and subspaces are typeset using calligraphic font.
% Superscripts are used for descriptive words \Ram{what does a descriptive word mean?}.
% Subscripts are used to follow conventional notations in the literature. 
Subscripts are primarily used as an index or to describe an particular coordinate of a vector.
% \subsection{Notations}
Let $\R$, $\R_+$ and $\N$ denote the spaces of real numbers, real positive numbers, and natural numbers, respectively.
% Let $[A,B]$ denote the concatenation of two matrices $A$ and $B$ with an identical number of rows.
% Let $0_{n_1\times n_2}$ denote the $n_1$-by-$n_2$ zero matrix.
% Denote $\|a\|_\infty$ the infinity norm of a vector $a\in\R^n$.
The Minkowski sum between two sets $\mathcal A$ and $\mathcal A'$ is $\mathcal A\oplus \mathcal A' = \{a+a'\mid a\in \mathcal A, ~a'\in \mathcal A'\}$.
Given a set $\mathcal A$, denote its power set as $P(\mathcal A)$ and its cardinality as $|\mathcal A|$.
% The power set of a set $\mathcal A$ is denoted by $P(\mathcal A)$.
Given vectors $\alpha,\beta\in\R^n$, let $[\alpha]_i$ denote the $i$-th element of $\alpha$, 
% let $\Sum(\alpha)$ denote the summation of all elements of $\alpha$, 
% let $\|\alpha\|$ denote the Euclidean norm of $\alpha$,
% Let $\diag(\alpha)$ denote the diagonal matrix with $\alpha$ on the diagonal, and 
and let $\Int(\alpha,\beta)$ denote the $n$-dimensional box $\{\gamma \in\R^n\mid [\alpha]_i\leq[\gamma]_i\leq[\beta]_i,~\forall i=1,\ldots,n\}$.
Given arbitrary matrix $A\in\R^{n_1\times n_2}$, let $[A]_{i:}$ denote the $i$-th row of $A$ for any $i\in\{1,2,\ldots,n_1\}$,
% let $A^\top$ be the transpose of $A$, 
% let $[A]_{i:}$ and $[A]_{:i}$ denote the $i$-th row and column of $A$ for any $i\in\{1,2,\ldots,n_1\}$ respectively, and 
% let $|A|$ be the matrix computed by taking the absolute value of every element in $A$.
and let $\det(A)$ be the determinant of $A$.
Let $\prob(\texttt E)$ denote the probability of occurrence of some event $\texttt E$.
Let $\pi_{xy}:\R^6\rightarrow\R^2$ be the projection operator that outputs the first two coordinates from its argument, and let $\rot(a)$ denote the 2-dimensional rotation matrix $\begin{bmatrix}
        \cos(a) & -\sin(a) \\ \sin(a) & \cos(a)
    \end{bmatrix}$ for arbitrary $a\in\R$.

Next, we introduce a subclass of polytopes, called zonotopes, that are used throughout this paper:
\begin{defn}
\label{def: zonotope}
A \emph{zonotope} $\Z$ is a subset of $\R^n$ defined as
\begin{equation}
    \mathcal Z = \left\{x\in\R^n\mid x= c+\sum_{k=1}^\ell \beta_k g_k, \quad \beta_k \in [-1,1] \right\}
\end{equation}
with \emph{center} $c\in\R^n$ and $\ell$ \emph{generators} $g_1,\ldots,g_\ell\in\R^n$.
% with center $c\in\R^n$ and $\ell$ generators $g^{(1)},\cdots,g^{(\ell)}\in\R^n$.
For convenience, we denote $\mathcal Z$ by $\zonocg{c}{G}$ where $G = [g_1, g_2, \ldots, g_\ell ]\in\R^{n\times\ell}$.
\end{defn}
\noindent Note that an $n$-dimensional box is a zonotope because
\begin{equation}
\label{eq: interval is zonotope}
    \Int(\alpha,\beta) = \zonocg{\frac{1}{2}(\alpha+\beta)}{\frac{1}{2}\diag(\beta-\alpha)}.    
\end{equation}
By definition the Minkowski sum of two arbitrary zonotopes  $\Z_1 = \zonocg{c_1}{G_1}$ and $\Z_2=\zonocg{c_2}{G_2}$ is still a zonotope as $\Z_1\oplus\Z_2 = \zonocg{c_1+c_2}{[G_1,G_2]}$.
Note that one can define the multiplication of a matrix $A$ of appropriate size with a zonotope $\Z=\zonocg{c}{G}$ as
\begin{equation}
\label{eq: zono-matrix mult}
   A \Z = \left\{x\in\R^n\mid x= A c+\sum_{k=1}^\ell \beta_k A g_k, ~ \beta_k \in [-1,1] \right\}.
\end{equation}
Note that $A \Z$ is equal to the zonotope $\zonocg{A c}{A G}$. 

% \challen{
% \section{Premiliminaries}
% \subsection{Notation}
% \subsection{Vehicle Dynamics and Trajectory Parameterization}
% \begin{itemize}
%     \item Open loop dynamics
%     \item Closed loop dynamics
%     \item Hybrid System definition
%     \item Trajectory Parameterization 
%     \item Ego vehicle definition (to be clear, just state and footprint definition)
% \end{itemize} 
% }

% \challen{
% \subsection{Environment}
% \begin{itemize}
%     \item 
%     \item Obstacle vehicle definition
%     \item State that there is uncertainty in obstacle vehicle observations and that uncertainty can be described as a probability and say it is formally defined in a later section
%     \item Sensing horizon  
% \end{itemize}
% }

% \challen{
% \subsection{Risk-Aware Vehicle Safety}
% \begin{itemize}
%     \item Not-at-fault definition 
% \end{itemize}
% }



% \challen{
% \section{Offline Reachability Analysis}
% \begin{itemize}
%     \item Assumption that there exists some collection of zonotopes that contain the vehicle trajectory, then we can introduce the reachable sets with simpler notation 
% \end{itemize}
% }

% \challen{
% \section{Online Planning and Chance Constraint}
% \subsection{Vehicle Dynamics and Trajectory Parameterization}
% \begin{itemize}
%     \item Obstacle Uncertainty
%     \item Online Optimization
%     \item Chance constraint relaxation
%     \item Enhanced Online Optimization  
% \end{itemize}
% }

\section{Preliminaries}

The goal of this work is to plan trajectories for an autonomous vehicle to navigate through environments with uncertainty in the locations of obstacles while having guarantees on the likelihood of collision.
We now discuss the vehicle model and dynamics, the parameterized trajectories and lastly the ego vehicle's environment.

\subsection{Open Loop Vehicle Dynamics}
\label{subsec: dynamics}

\subsubsection{High-Speed Model}
\label{subsubsec: vehicle}
This work adopts the Front-Wheel-Drive vehicle model and control from \cite{REFINE}.
Note that the approach could be generalized to an all wheel or rear wheel drive models just as is done in \cite{REFINE}.
Let the ego vehicle's states at a time  $t$ be given by $\zhi(t) = [x(t),y(t),h(t),u(t),v(t),r(t)]^\top\in \R^6$, where $x(t)$ and $y(t)$ are the position of the ego vehicle's center of mass in the world frame, $h(t)$ is the heading of the ego vehicle in the world frame, $u(t)$ and $v(t)$ are the longitudinal and lateral speeds of the ego vehicle in its body frame, and $r(t)$ is the yaw rate of the vehicle center of mass.
To simplify exposition, we assume vehicle weight is uniformly distributed and ignore the aerodynamic effect while modeling the flat ground motion of the vehicles by the following dynamics:
\begin{align}
    \label{eq:dynamics_hi}
    \dzhi(t) & = 
    \begin{bmatrix}
        u(t)\cos h(t) - v(t)\sin h(t)\\ u(t)\sin h(t) + v(t)\cos h(t) \\ r(t)\\
        \frac{1}{m}\big(F_\text{xf}(t)+F_\text{xr}(t)\big) + v(t)r(t) + \Delta_u(t) \\ 
        \frac{1}{m}\big(F_\text{yf}(t)+F_\text{yr}(t)\big)-u(t)r(t)+ \Delta_v(t)\\
        \frac{1}{I_\text{zz}} \big(l_\text{f} F_\text{yf}(t) - l_\text{r} F_\text{yr}(t)\big)+ \Delta_r(t)
    \end{bmatrix}. 
    % \dot z_\text{lo}(t) &= \pi_4(\dot z_\text{hi}(t)). \label{eq:lowspeed_noise}
\end{align}
where $l_\text{f}$ and $l_\text{r}$ are the distances from center of mass to the front and back of the vehicle, $I_\text{zz}$ is the vehicle's moment of inertia, and $m$ is the vehicle's mass.
Note: $l_\text{f}$, $l_\text{r}$, $I_\text{zz}$ and $m$ are all constants and are assumed to be known.
The tire forces along the longitudinal and lateral directions of the vehicle at time $t$ are $F_\text{xi}(t)$ and $F_\text{yi}(t)$ respectively, where the `i' subscript can be replaced by `f' for the front wheels or `r' for the rear wheels. 
$\Delta_u,\Delta_v,\Delta_r$ are modeling error signals that are unknown and account for imperfect state estimation and inaccurate tire models.
To ensure the system is well-posed (i.e., its solution exists and is unique), we make the following assumption:
\begin{assum}
\label{ass: dyn error bnd}
    $\Delta_u, \Delta_v,\Delta_r$ are all square integrable functions and are bounded (i.e., there exist real numbers $M_u, M_v, M_r\in [0,+\infty)$ such that $\|\Delta_u(t)\|_\infty\leq M_u, ~\|\Delta_v(t)\|_\infty\leq M_v, ~\|\Delta_r(t)\|_\infty \leq M_r$ for all $t$).
\end{assum}
\noindent Note that $\Delta_u,\Delta_v,\Delta_r$ can be computed using real-world data \cite[Section IX-C]{REFINE}.

In this work we assume linear tire models and assume that we can directly control the front tire forces, $F_\text{xf}$ and $F_\text{yf}$. 
Such assumptions are validated in \cite[Section V.B and VIII.B]{REFINE}.
Additionally we treat rear tire forces as observed signals. 
% Unfortunately, in the real-world our state estimation and models for front and rear tire forces may be inaccurate and aerodynamic-drag force could also affect vehicle dynamics \cite[Section 4.2]{ulsoy2012automotive}.
% To account for the inaccuracy, we introduce time-varying affine modeling error terms $\Delta_u,\Delta_v,\Delta_r$ into the dynamics of $u,v,$ and $r$ as shown in \eqref{eq:dynamics_hi}.

% To ensure that this definition is well-posed (i.e. their solution exists and is unique) and to aid in the development of our controller as described in Section \ref{subsec:cl-dynamics}, we make the following assumption:
% \begin{assum}
% \label{ass: dyn error bnd}
%     $\Delta_u, \Delta_v,\Delta_r$ are all square integrable functions and are bounded (i.e., there exist real numbers $M_u, M_v, M_r\in [0,+\infty)$ such that $\|\Delta_u(t)\|_\infty\leq M_u, ~\|\Delta_v(t)\|_\infty\leq M_v, ~\|\Delta_r(t)\|_\infty \leq M_r$ for all $t$).
% \end{assum}
% \noindent Note that $\Delta_u,\Delta_v,\Delta_r$ can be computed using real-world data \cite[Section IX-C]{REFINE}.

\subsubsection{Low-Speed Model}
When the vehicle speed lowers below some critical value $\uc>0$, applying the model described in \eqref{eq:dynamics_hi} becomes intractable as explained in \cite[Section III-B]{REFINE}. 
As a result, in this work when $u(t)\leq \uc$, the dynamics of a vehicle are modeled using a steady-state cornering model \cite[Chapter 6]{gillespie1992fundamentals}, \cite[Chapter 5]{balkwill2017performance}, \cite[Chapter 10]{dieter2018vehicle}.
Note that the critical velocity $\uc$ can be found according to \cite[(5) and (18)]{kim2019advanced}.

The steady-state cornering model or low-speed vehicle model is described using four states, $\zlo(t) = [x(t),y(t),h(t),u(t)]^\top\in\R^4$ at time $t$.
This model ignores transients on lateral velocity and yaw rate. 
Note that the dynamics of $x$, $y$, $h$ and $u$ in the low-speed model are the same as in the high-speed model \eqref{eq:dynamics_hi}; however, the steady-state cornering model describes the yaw rate and lateral speed as
\begin{align}
    \vlo(t) =&l_\text{r}\rlo(t) - \frac{ml_\text{f}}{\bar c_{\alpha\text{r}}l}u(t)^2\rlo(t)   \label{eq: v lo} \\
    \rlo(t) =& \frac{\delta(t)u(t)}{l+C_\text{us} u(t)^2} \label{eq: r lo}
\end{align}
with understeer coefficient
\begin{equation}
    C_\text{us} = \frac{m}{l}\left( \frac{l_\text{r}}{\bar c_{\alpha \text{f}}} - \frac{l_\text{f}}{\bar c_{\alpha \text{r}}} \right),
\end{equation}
where $\delta(t)$ is the steering angle of the front tire at time $t$, $\bar c_{\alpha \text{f}}$ and $\bar c_{\alpha \text{r}}$ are cornering stiffness of the front and rear tires respectively. 
% As a result, $\dzlo$ satisfies the dynamics of the first four states in \eqref{eq:dynamics_hi} except with $\rlo$ taking the role of $r$ and $\vlo$ taking the role of $v$.

As we describe in detail in Section \ref{subsec:cl-dynamics}, the high-speed and low-speed models can be combined together as a hybrid system to describe the behavior of the vehicle across all longitudinal speeds. 
In short, when $u$ transitions past the critical speed $\uc$ from above at time $t$, the low speed model's states are initialized as:
\begin{equation}
\label{eq: reset h2l}
    \zlo(t) = \pi_{1:4}(\zhi(t))
\end{equation}
where $\pi_{1:4}:\R^6\rightarrow\R^4$ is the projection operator that projects $\zhi(t)$ onto its first four dimensions via the identity relation.
If $u$ transitions past the critical speed from below at time $t$, the high speed model's states are initialized as
\begin{equation}
\label{eq: reset l2h}
    \zhi(t) = [\zlo(t)^\top, \vlo(t), \rlo(t)]^\top.
\end{equation}


\subsection{Trajectory Parameterization}

Each trajectory plan is specified over a compact time interval. 
% Without loss of generality, we let each plan begin at time $\tz$ and end at a fixed final time $\tf$.
Without loss of generality, we let this compact time interval have a fixed duration $\tf$.
Because $\riskmethodname{}$ performs receding-horizon planning, we make the following assumption about the time available to construct a new plan:
\begin{assum} \label{assum:tplan}
During each planning iteration starting from time $\tz$, the ego vehicle has $\tplan$ seconds to find a control input.
This control input is applied during the time interval $[\tz+\tplan, \tz+\tplan+\tf]$ where $\tf \geq 0$ is a user-specified constant. 
In addition, the state of the vehicle at time $\tz+\tplan$ is known at time $\tz$. 
% \jinsun{do we want to weaken the last sentence by introducing prediction error?}
\end{assum}
\noindent This assumption requires \riskmethodname{} to generate plans in a real-time fashion.
This means that the ego vehicle must create a new plan before it finishes executing its previously planned trajectory.

In each planning iteration, \riskmethodname{} chooses a trajectory to be followed by the ego vehicle.
These trajectories are chosen from a pre-specified continuum of trajectories, with each uniquely determined by a \textit{trajectory parameter} $p \in \P$.
Let $\P \subset \R^{n_p}$, $n_p \in \N$ be a n-dimensional box $\Int(\underline p, \overline p)$ where $\underline p, \overline p\in\R^{n_p}$ indicate the element-wise lower and upper bounds of $p$, respectively.
We define these desired trajectories as follows:
% We say that $k \in K$ maps to a desired trajectory $q_d(\cdot; k) : T \to \Q$, and use $\qdesk$ to denote the configuration along this trajectory parameterized by $k$ at time $t$.

\begin{defn}\label{def:traj_param}
For each $p \in \P$, a \emph{desired trajectory} is a function for the longitudinal speed, $\udes(\cdot,p):[\tz+\tplan,\tz+\tplan+t_\text{f}] \to \R$, a function for the heading, $\hdes(\cdot,p):[\tz+\tplan,\tz+\tplan+t_\text{f}] \to \R$, and a function for the yaw rate, $\rdes(\cdot,p): [\tz+\tplan,\tz+\tplan+t_\text{f}] \to \R$, that satisfy the following properties.
\begin{enumerate}
% We require that $q_d(\cdot; k): T \to Q$ satisfies three properties for all $k \in K$
\item For all $p\in\P$, there exists a time instant $\tnb\in[\tz+\tplan,\tz+\tplan+\tf)$ after which the desired trajectory begins to brake (i.e., $|\udes(t,p)|$, $|\hdes(t,p)|$ and $|\rdes(t,p)|$ are non-increasing for all $t\in[\tnb,\tz+\tplan+\tf]$).
\item The desired trajectory eventually comes to and remains stopped (i.e., there exists a $\tstop \in [\tz+\tplan,\tz+\tplan+\tf]$ such that $\udes(t, p) = \hdes(t, p) = \rdes(t, p) = 0$ for all $t \geq \tstop$).
\item $\udes$ and $\hdes$ are piecewise continuously differentiable \cite[Chapter 6, $\S$1.1]{remmert1991theory} with respect to $t$ and $p$.
\item The time derivative of the heading function is equal to the yaw rate function (i.e., $\rdes(t,p)=\frac{\partial}{\partial t}\hdes(t,p)$ over all regions that $\hdes(t,p)$ is continuously differentiable with respect to $t$).
% \item $q_d(\cdot; k) $ is at least once-differential with respect to time (i.e., no discontinuities in joint position or velocity).
% \pat{Third, $q(0; k) = 0$ (each joint starts from zero initial angle).}
\end{enumerate}
\end{defn}
\noindent The first two properties ensure that a fail safe maneuver is always available due to the safety concern as described later in Section \ref{subsec: risk-aware safety}, and the latter two properties ensure that the tracking controller described in Section \ref{subsec:cl-dynamics} is well-defined.
Note that sometimes we abuse notation and evaluate a desired trajectory for $t > \tf$.
In this instance, the value of the desired trajectory is equal to its value at $\tf$.
In addition, for simplicity we call the portion of a desired trajectory during $[\tz+\tplan,\tz+\tplan+\tm)$ \emph{the driving maneuver} and during  $[\tz+\tplan+\tm,\tz+\tplan+\tf]$ \emph{the contingency braking maneuver}.

\subsection{Closed Loop Vehicle Dynamics}
\label{subsec:cl-dynamics}
This subsection describes the controller and closed-loop hybrid system vehicle model. 
We start by introducing the controller on longitudinal speed whose dynamics appears in both high-speed and low-speed models as done in \cite[Section V-A]{REFINE}.
We set the longitudinal front tire force to be:
\begin{equation}
    \label{eq: Fxf}
    \begin{split}
    F_\text{xf}(t) = -m K_u (u(t) - \udes(t,p) ) + m\dudes(t,p) + \\ - F_\text{xr}(t)- mv(t)r(t) + m\tau_u(t,p),
    \end{split}
\end{equation}
where
\begin{align}
\tau_u(t,p) =& -\big(\kappa_u(t,p) M_u+\phi_u(t,p)\big)e_u(t,p), \label{eq: tau_u def} \\
    \kappa_u(t,p) =& \kappa_{1,u}+\kappa_{2,u}\int_{\tz}^t\|u(s)-\udes(s,p)\|^2ds,\label{eq: kappa_u def}\\
    \phi_u(t,p) =&\phi_{1,u}+\phi_{2,u}\int_{\tz}^t\|u(s)-\udes(s,p)\|^2ds,\label{eq: phi_u def}\\
    e_u(t,p) =& u(t)-\udes(t,p), \label{eq: e_u def}
\end{align}
with user-chosen constants $K_u,\kappa_{1,u},\kappa_{2,u},\phi_{1,u},\phi_{2,u}\in\R_+$.
Note in \eqref{eq: Fxf} we have suppressed the dependence on $p$ in $F_\text{xf}(t)$ for notational convenience.
Using \eqref{eq: Fxf}, the closed-loop dynamics of $u$ become: 
\begin{equation}
\begin{split}
    \dot u(t) = \tau_u(t,p) + \Delta_u(t) + \dudes(t,p) + \\ -K_u \left( u(t) - \udes(t,p)\right).
    \end{split}
    \label{eq: u_dot_closed_loop_eq}
\end{equation}

The same control strategy can be applied to vehicle yaw rate whose dynamics only appear in  the high-speed vehicle model.
Let the lateral front tire force be 
\begin{equation}
\label{eq: Fyf}
\begin{split}
    % F_\text{yf}(t) = \frac{1}{l_\text{f}}\big(I_\text{zz}\drexp(t,p)+ l_\text{r}F_\text{yr}(t) + I_\text{zz}\varphi_r(t,p) \big)
     F_\text{yf}(t) = -\frac{I_\text{zz} K_r}{l_\text{f}}\left( r(t) - \rdes(t,p) \right) +  \frac{I_\text{zz}}{l_\text{f}} \drdes(t,p) + \\ -\frac{I_\text{zz} K_h}{l_\text{f}}\left( h(t) - \hdes(t,p)\right) + \frac{l_\text{r}}{l_\text{f}} F_\text{yr}(t) + \frac{I_\text{zz}}{l_\text{f}} \tau_r(t,p),
     \end{split}
    % \frac{I_\text{zz}}{l_\text{f}}\drexp(t;d) +\frac{l_\text{r}}{l_\text{f}} F_\text{yr}(t) + \frac{I_\text{zz}}{l_\text{f}}\varphi_r(t;d)
\end{equation}
where
\begin{align}
 \tau_r(t,p) =& -\big(\kappa_r(t,p) M_r+\phi_r(t,p)\big)e_r(t,p) \label{eq: tau_r def} \\
    \kappa_r(t,p) =& \kappa_{1,r}+\kappa_{2,r}\int_{\tz}^t\left\| \begin{bmatrix}r(s)\\h(s)\end{bmatrix} - \begin{bmatrix}\rdes(s,p)\\\hdes(s,p)\end{bmatrix}\right\|^2ds\\
    \phi_r(t,p) =&\phi_{1,r}+\phi_{2,r}\int_{\tz}^t\left\| \begin{bmatrix}r(s)\\h(s)\end{bmatrix} - \begin{bmatrix}\rdes(s,p)\\\hdes(s,p)\end{bmatrix}\right\|^2ds\\
    % e_r(t,p) =& K_r(r(t)-\rdes(t,p))+K_h(h(t)-\hdes(t,p)),
    e_r(t,p) =& \begin{bmatrix} K_r & K_h \end{bmatrix} \begin{bmatrix} r(t)-\rdes(t,p) \\ h(t)-\hdes(t,p) \end{bmatrix}
\end{align}
with user-chosen constants $K_h,K_r,\kappa_{1,r},\kappa_{2,r},\phi_{1,r},\phi_{2,r}\in\R_+$.
Note in \eqref{eq: Fyf} we have again suppressed the dependence on $p$ in $F_\text{yf}(t)$ for notational convenience.
Using \eqref{eq: Fyf}, the closed-loop dynamics of $r$ become:
\begin{equation}
    \begin{split}
    \dot r(t) = &\tau_r(t,p)+ \Delta_r(t)+ \drdes(t,p) + \\ & -K_r\big(r(t) - \rdes(t,p)\big)+  \\  &-K_h\big(h(t) - \hdes(t,p)\big).
    \end{split}
    \label{eq: r_dot_closed_loop_eq}
\end{equation}
Using \eqref{eq: Fyf}, the closed-loop dynamics of $v$ become:
\begin{equation}
    \begin{split}
        \dot v(t) = \frac{1}{m}\Bigg(\frac{l}{l_\text{f}} F_\text{yr}(t) +\frac{I_\text{zz}}{l_\text{f}}\Big(\tau_r(t,p) + \drdes(t,p) + \\
        - u(t)r(t)+\Delta_v(t) -K_r\big(r(t) - \rdes(t,p)\big) + \\ -K_h\big(h(t) - \hdes(t,p)\big) \Big) \Bigg).
    \end{split}
    \label{eq: v_dot_closed_loop_eq}
\end{equation}

Because $\udes$, $\rdes$, and $\hdes$ depend on trajectory parameter $p$, one can rewrite the closed loop high-speed and low-speed vehicle models as
\begin{align}
    \dzhi(t) &= \fhi(t,\zhi(t),p), \label{eq: hi_veh_closeloop}\\
    \dzlo(t) &= \flo(t,\zlo(t),p), \label{eq: lo_veh_closeloop}
\end{align}

\noindent Moreover, because the vehicle's dynamics changes depending on $u$, it is natural to model the ego vehicle as a hybrid system $HS$  \cite[Section 1.2]{lunze2009handbook} as done in \cite[Section V-C]{REFINE}.
The hybrid system $HS$ contains a high-speed mode and a low-speed mode with state $z:=\zhi$, whose dynamics can be written as 
\begin{equation}
\label{eq: dyn tilde_z}
    z(t) = \begin{dcases}
            \fhi(t,\zhi(t),p) , \text{ if } u(t) > \uc, \\ \\
        \begin{bmatrix}
            \flo(t,\zlo(t),p) \\ 0_{2\times1}
        \end{bmatrix} , \text{ if } u(t) \leq \uc,
    \end{dcases}
\end{equation}
Instantaneous transition between the two modes within $HS$ are described using the notion of a \emph{guard} and \emph{reset map}.
The guard triggers a transition and is defined as $\{z(t)\in\R^{6}\mid u(t) =\uc\}$. 
Once a transition happens, the reset map resets the first $z(t)$ via \eqref{eq: reset h2l} if $u(t)$ approaches $\uc$ from above and via \eqref{eq: reset l2h} if $u(t)$ approaches $\uc$ from below. 



% \jinsun{I think we can avoid introducing $\zaug$ completely because it's only for offline reachability analysis. And I'm defining the hybrid system with non-augmented states.}\strikethrough{In addition, for computational reasons that are described in \cite[Section VI]{REFINE} , we augment the initial condition of the system to the state vector while describing the vehicle dynamics.
% In particular, denote $z_0 = [(\zpos_0)^\top, (\zvel_0)^\top]^\top\in\Z_0\subset\R^6$ the initial condition of the ego vehicle where $\zpos_0=[x_0,y_0,h_0]^\top\in\R^3$ gives the value of $[x(t),y(t),h(t)]^\top$ and $\zvel_0=[u_0,v_0,r_0]^\top\in\R^3$ gives the value of $[u(t),v(t),r(t)]^\top$ at time $t=0$.
% Then we augment the initial velocity condition $\zvel_0\in\R^3$ of the vehicle model and trajectory parameter $p$ into the vehicle state vector as $\zaug(t) = [x(t),y(t),h(t),u(t),v(t),r(t), (\zvel_0)^\top, p^\top]^\top\in\R^{9}\times\P\subset\R^{9 + n_p}$.
% Note the last $3 + n_p$ states are static with respect to time.
% As a result, the dynamics of the augmented vehicle state during high-speed and low-speed scenarios can be written as}
% \begin{equation}
% \label{eq: dyn tilde_z_bla}
%     \dzaug(t) = \begin{dcases}
%         \begin{bmatrix}
%             \fhi(t,\zhi(t),p) \\ 0_{ (3 + n_p) \times1}
%         \end{bmatrix} , \text{ if } u(t) > \uc, \\ \\
%         \begin{bmatrix}
%             \flo(t,\zlo(t),p) \\ 0_{(5 + n_p)\times1}
%         \end{bmatrix} , \text{ if } u(t) \leq \uc,
%     \end{dcases}
% \end{equation}
% \strikethrough{which we refer to as the \emph{hybrid vehicle dynamics model}.
% Notice when $u(t)\leq \uc$, assigning zero dynamics to $v$ and $r$ in \eqref{eq: dyn tilde_z} does not affect the evolution of the vehicle's dynamics because the lateral speed and yaw rate are directly computed via longitudinal speed as in \eqref{eq: v lo} and  \eqref{eq: r lo}.

% The hybrid system has $\zaug$ as its state and consists of a high-speed mode and a low-speed mode with dynamics in \eqref{eq: dyn tilde_z}.
% Instantaneous transition between the high and low speed models within $HS$ are described using the notion of a \emph{guard} and \emph{reset map}.
% The guard triggers a transition and is defined as $\{\zaug(t)\in\R^{9}\times\P\mid u(t) =\uc\}$. 
% Once a transition happens, the reset map maintains the last $3+n_p$ dimensions of $\zaug(t)$, but resets the first $6$ dimensions of $\zaug(t)$ via \eqref{eq: reset h2l} if $u(t)$ approaches $\uc$ from above and via \eqref{eq: reset l2h} if $u(t)$ approaches $\uc$ from below. }

\subsection{Ego Vehicle, Environment, and Sensing}
\label{subsec: environment}
To provide guarantees about vehicle behavior in a receding horizon planning framework we define the ego vehicle's footprint similarly to \cite[Definition 10]{REFINE}:

\begin{defn}
\label{def: footprint}
Given $\W\subset\R^2$ as the world space, the ego vehicle is a rigid body that lies in a rectangle $\mathcal O^{ego}:=\Int([-0.5L,-0.5W]^T,[0.5L,0.5W]^T )\subset\W$ with width $W>0$ and length $L>0$ at time $t=0$. 
$\mathcal O^{ego}$ is called the \emph{footprint} of the ego vehicle.
\end{defn}
\noindent For arbitrary time $t$, given state $z(t)$ of the ego vehicle that starts from initial condition $z_0\in\Z_0\subset\R^6$ and applies a control input parameterized by $p\in\P$, the ego vehicle's footprint at time $t$ can be represented as
\begin{equation}
    \hspace{-0.2cm}\E\big(t,z_0,p\big) := \rot(h(t))\cdot\Oego + [x(t),y(t)]^\top,
\end{equation}
% \jinsun{I don't like this notation because if $z(t)$ is known, then why $z_0$ and $p$ are necessary? I'd suggest $\E(t,z_0,p)$.}
which is a zonotope by \eqref{eq: zono-matrix mult}.
% \subsection{Environment}
% \label{subsec: environment}
% \ram{why is the ego vehicle's footprint in the environment section?} \challen{resolved}
We define the obstacles in the following way:
\begin{defn}
% Let $\O\Oobs(t)$ be the location of an obstacle given according to sensor measurements at time $t$, where $i\in\I$ is the index of the obstacle and $\I$ contains finitely many elements. 
% \challen{maybe we should move Assumption 6 to the beginning of this section, and reframe it st we define ]$\Oest$ inside of it.}
An \emph{obstacle} is a set $\Oobs(t)\subset \W$ that the ego vehicle should not collide with at time $t$, where $i\in\I$ is the index of the obstacle and $\I$ contains finitely many elements. 
Let the footprint of the obstacle 
% Let $\cobs(t)\in\W$ be the center of $\Oobs(t)$. 
\end{defn}

\noindent The dependency on $t$ in the definition of an obstacle allows the obstacle to move as $t$ varies. 
However if the $i$-th obstacle is static, then $\Oobs(t)$ is a constant.
Note that in this work, we assume that we do not have perfect knowledge of obstacle locations and motion as is normally the case in real-life scenarios.
We assume that this uncertainty in the obstacles locations is represented by some arbitrary probability distribution. 
We formally discuss its representation in the next section.
Assuming that the ego vehicle has a maximum speed $\vegomax$ and all obstacles have a maximum speed $\vobsmax$ for all time, we then make the following assumption on planning and sensing horizon. 
\begin{assum}
\label{ass: sense horizon}
The ego vehicle senses all obstacles within a sensor radius $S>(\tf +\tplan)\cdot(\vegomax+\vobsmax)+0.5\sqrt{L^2+W^2}$ around its center of mass.
\end{assum}
\noindent Assumption \ref{ass: sense horizon} ensures that any obstacle that can cause a collision between times $t\in[\tz+\tplan, \tz+\tplan+\tf]$ can be detected by the vehicle \cite[Theorem 15]{vaskovtowards}.
Note one could treat sensor occlusions as obstacles that travel at the maximum obstacle speed \cite{yu2019occlusion,yu2020risk}.
% Lastly, to account for uncertainty in the locations of obstacles caused by imperfect sensing of obstacles due to sensor noise, or imperfect prediction of obstacle motion, one can represent the obstacle location as a probability distribution. 
% In Section \ref{subsec:obs uncertainty}, we formally define the properties of this probability distribution. 
To simplify notation, we reset time to $0$ whenever a feasible control policy is about to be applied, \emph{i.e.}, $t_0+\tplan = 0$.
Finally to aid in the descriptions of obstacle uncertainty and system trajectory over-approximation in Sections \ref{sec:online planning} and \ref{sec:risk-rtd and reachability analysis}, we partition the planning horizon $[0,\tf]$ into $\tf/\Delta_t$ \emph{time intervals} with some positive number $\Delta_t$ that divides $\tf$, and denote $T_j$ the $j$-th time interval $[(j-1)\Delta_t, j\Delta_t]$ for any $j\in \J:=\{1,2,\ldots,\tf/\Delta_t\}$.



% \subsection{Receding Horizon Planning and Timing}

% \riskmethodname{} plans in a receding horizon format, meaning that it generates a plan and has the entire plan executed while generating the next plan. 
% Each plan is specified over a compact time interval with a fixed duration $\tf$, and we make the following assumption about the time needed to construct a new plan.  

% \begin{assum} \label{assum:tplan}
% During each planning iteration starting from time $\tz$, the ego vehicle has $\tplan$ seconds to find a control input.
% This control input is applied during the time interval $[\tz+\tplan, \tz+\tplan+\tf]$ where $\tf \geq 0$ is a user-specified constant. 
% In addition, the state of the vehicle at time $\tz+\tplan$ is known at time $\tz$. 
% \end{assum}

% % \Ram{the remainder of this section seems as if its in the wrong place as it requires a lot of information about FRS-es, and how planning works. Probably it should live after the relevant objects have been defined. 
% % For instance you break things into time segments, but provide no rationale for doing that...}
% Assuming that the ego vehicle has a maximum speed $\vegomax$ and all obstacles have a maximum speed $\vobsmax$ for all time, we then make the following assumption on planning and sensing horizon. 
% \begin{assum}
% \label{ass: sense horizon}
% The ego vehicle senses all obstacles within a sensor radius $S> (\tf +\tplan)\cdot(\vegomax+\vobsmax)+0.5\sqrt{L^2+W^2}$ around its center of mass.
% \end{assum}

% Assumption \ref{ass: sense horizon} ensures that any obstacle that can cause a collision between times $t\in[t_0 + \tplan, t_0 + \tplan+\tf]$ can be detected by the vehicle \cite[Theorem 15]{vaskovtowards}. 
% \Ram{what about occlusions?} \new{Note one could treat sensor occlusions as a obstacles that travel at the maximum obstacle speed \cite{yu2019occlusion,yu2020risk}.}
% % Without loss of generality (WLOG), since time can be shifted to $0$ at the beginning of each plan, we can denote $T = [0, \tf]$ as the time horizon for a single plan executed between  $[\tz+\tplan, \tz+\tplan+\tf]$.
% To simplify notation, we reset time to 0 whenever a feasible control policy is about to be applied, i.e. $t_0+\tplan = 0$.

% % It is also important to note that after a feasible plan is found, time is reset to 0 such that in the vehicle's local time frame the maneuvers are executed in the time interval $[0, \tf]$.
% % Next we pick a time step $\Delta_t\in\R_+$ such that $\tf/\Delta_t\in\N$, and partition the time interval $[0,\tf]$ into $\tf/\Delta_t$ \emph{time segments} as $T_j=[(j-1)\Delta_t, j\Delta_t]$ for each $j\in \J=\{1,2,\cdots,\tf/\Delta_t\}$. 

% \Ram{the portion of this paragraph related to braking maneuvers probably should appear when you describe the trajectory parameterization.}
% Lastly, we append a braking maneuver to all reference trajectories parameterized by $p$ so that the vehicle can come to a safe stop if it is unable to find a feasible path plan during operation. 
% This allows us to ensure that the vehicle not-at-fault in these situations.
% Recall that time can be reset such that the vehicle vehicle performs its planned maneuver in the time interval  $[0, \tf]$. 
% This interval can be further broken up into a driving maneuver part,  $[0, \tm]$ and a braking maneuver part  $[\tm, \tf]$ where $\tm$ is the duration of the planned maneuver execution \cite{REFINE}.
% We further enforce that $\tplan \leq \tm$ to ensure real-time performance.
% Note that each reference trajectory given by $p$ has a braking maneuver appended to it. 
% \jinsun{maybe consider to swap the last two subsections and append this paragraph (need to be polished) to the receding `horizon planning section'? Also need to say $\tplan \leq \tm$ for real-time performance}



% \begin{equation}
% \label{eq: chance constraint}
%     \color{cyan} \prob\bigg(\Big(\cup_{t\in[0,\tf]}\E\big(z(t),z_0,p\big)\Big) \cap \big(\cup_{i\in\Irisk}\Oest_i(t)\big)\neq\emptyset \bigg) \leq \epsilon
% \end{equation}



==> sections_long/04_online_planning.tex <==
\section{Online Planning Under Uncertainty}
\label{sec:online planning}
% We now describe how \riskmethodname{} seeks a feasible not-at-fault plan online. 

This section constructs a chance-constrained optimization problem to generate risk-aware motion plans. 
First, we describe the representations of the obstacle uncertainty used in this work. 
Then, we define risk-aware vehicle safety and conclude by illustrating how to formulate online planning as a chance-constrained optimization that limits the risk of collision.

\subsection{Obstacle Uncertainty}
\label{subsec:obs uncertainty}
To incorporate the uncertainty in both the obstacle sensing and obstacle motion prediction into the motion planning framework, let $\wobs$ be a random variable that takes values in $\W$.
In particular, $\wobs$ describes the possible locations of the center of the $i$-th obstacle, $\Oobs(t)$, for any time $t\in T_j$.
We then make the following assumption about how $\wobs$ is distributed:

\begin{assum}
\label{ass: obs pdf}
    % For any $i\in\I$ and $j\in\J$, there exists a function $f:\W\times\I\times\J\rightarrow\R_+$ such that $\int_\W f(w) ~dw = 1$ and $f(w)$ gives the probability density of a point $w\in\W$ appears inside $\Oobs(t)$ at any time $t\in T_j$. 
    % For any $(i,j)\in\J\times\I$, there exists a probability density function $f$ such that $f(w)$ gives the probability density of a point $w\in\W$ belonging to $\cup_{t\in T_j}\Oobs(t)$. 
    % Moreover, $f$ is continuous and differentiable with respect to $w$.
    % The location $\Oobs(t)$ of the $i$-th obstacle at some $t \in T_j$ is given by a continuous and at least twice-differentiable probability distribution from an exponential family.
    For any $i\in\I$ and $j\in\J$, $\wobs$'s 
    % \strikethrough{let $\wobs := \cobs((j-0.5)\Delta t)$. $\wobs$ is a random variable with a probability density function $\pdf(\cdot\mid i,j):\W\rightarrow [0,+\infty)$. The probability density function $\pdf$ is twice-differentiable.}
    % \new{the probability distribution of $\wobs := \cobs((j-0.5)\Delta_t)$ satisfies a twice-differentiable probability density function $\pdf(\cdot):\W\rightarrow [0,+\infty)$.}
    % and draws from some probability distribution in the exponential family. \jinsun{the sentences don't make sense}\challen{better now?} 
    % \strikethrough{For any $i\in\I$ and $j\in\J$, $\cup_{t\in T_j} \Oobs(t)$ stays inside a zonotope $\zonocg{\w}{\Gobs}\subset\W$ where $\Gobs$ is a 2-row matrix that accounts for the volume swept by $\Oobs(t)$ over the time interval $T_j$.  
    % $\w\in\W$ satisfies a probability distribution from an exponential family with probability density $f(\w)\in [0,+\infty)$.
    % The probability density function $f$ is further assumed to be continuous and at least twice-differentiable with respect to $w$. 
    probability density function, $\pdf:\W\rightarrow[0,+\infty)$,  exists and is twice-differentiable.
    % \new{the distribution of $\wobs$ admits some probability density function $\pdf:\W\rightarrow[0,+\infty)$ that is Lebesgue-integrable and twice-differentiable.} \jinsun{note I no longer use notation $q(\cdot\mid i,j)$ to avoid the potential misleading to conditional probability, especially in the case where our $i$ and $j$ are not random variables at all.}
\end{assum}
% \noindent We let $\prob_{i,j}$ denote the probability distribution function associated with $\pdf$.

To account for the obstacle's footprint, we make the following assumption:
\begin{assum}
\label{ass: swept_volume assumption}
There exists a 2-row matrix $\Gobs$ such that
% \strikethrough{$\cup_{t\in T_j} \Oobs(t)$ stays inside a zonotope $\zonocg{\wobs}{\Gobs}\subset\W$ for all $(i,j)\in\I\times\J$.}
$\Oobs(t)\subseteq\zonocg{\wobs}{\Gobs}$ for all $i\in\I$, $j\in\J$, and $t \in T_j$.
\end{assum}

\noindent According to Assumptions \ref{ass: obs pdf} and \ref{ass: swept_volume assumption}, $\zonocg{\wobs}{\Gobs} = \wobs+\zonocg{0}{\Gobs}$ has an uncertain center $\w$ with probability density $\pdf(\w)$, and has invariant shape and size with respect to $i$ and $j$ due to the constant generator matrix $\Gobs$.
Such probability density functions $\pdf$ can be generated by, for example, performing variants of Kalman Filter \cite{vel_EKF_zindler,almeida2013real} on the $i$-th obstacle given its dynamics or detecting the $i$-th obstacle with a Bayesian confidence framework \cite{fisac2018probabilistically} during $T_j$.
The generator matrix $\Gobs$ can be generated as the union of footprints of all obstacles. 


% \cite{kalman1960new,ribeiro2004kalman,wan2000unscented}

\subsection{Risk-Aware Vehicle Safety}
\label{subsec: risk-aware safety}
In dynamic environments, it may be difficult to avoid collisions in all scenarios (\emph{e.g.}, a parked ego vehicle can be run into). 
As a result, we instead develop a trajectory synthesis technique that ensures that the ego vehicle is not-at-fault \cite[Definition 11]{vaskovtowards}.
We define not-at-fault safety in this work from a probabilistic perspective by bounding the probability of the ego vehicle running into any obstacles.
\begin{defn}\label{defn:notatfault-risk}
Let the ego vehicle start from initial condition $z_0\in\Z_0$ with control parameter $p\in\P$.
% Let the risk threshold be the maximum allowable probability of collision between the ego vehicle and all obstacle vehicles for a given motion plan.
Given a user-specified \emph{allowable risk threshold} $\epsilon\in[0,1]$, the ego vehicle is \emph{not-at-fault}, with a chance of collision of at most $\epsilon$, if it is stopped, or if 
% \begin{equation}
%     \stkout{\prob\bigg(\cup_{t\in[0,\tf]}\Big(\E\big(t,z_0,p\big) \cap \big(\cup_{i\in\I}\Oobs(t)\big) \Big)  \bigg) \leq \epsilon }   
% \end{equation}
\begin{equation}
    \label{eq: chance constraint def}
    % \sum_{i\in\I}\sum_{j\in\J} \prob_{i,j}\Big( \cup_{t\in T_j} \big( \E(t,z_0,p) \oplus \Gobs \big) \Big) \leq \epsilon,
     \sum_{i\in\I}\sum_{j\in\J}\int_{ \cup_{t\in T_j} \left( \E(t,z_0,p)\oplus\zonocg{0}{\Gobs} \right)} \pdf(w) ~dw \leq \epsilon,
\end{equation}
% \begin{equation}
%    \label{eq: chance constraint def}
%     \new{\prob\big( \{t\in[0,\tf]\mid\E(t,z_0,p)\cap\cup_{i\in\I}\Oobs(t)\}\neq\emptyset \big) \leq \epsilon }   
% \end{equation}
% \begin{equation}
%    % \label{eq: chance constraint def}
%     \challen{\prob\big( \wobs \in \E(t,z_0,p)\oplus\zonocg{0}{\Gobs} \mid t\in[0,\tf], i \in \I \big)}
% \end{equation}
while it is moving during $[0,\tf]$.
\end{defn}
\noindent \Ram{maybe add a sentence to explain what \eqref{eq: chance constraint def} means?} Note in particular that the domain of integration in \eqref{eq: chance constraint def} $\cup_{t\in T_j} \left( \E(t,z_0,p)\oplus\zonocg{0}{\Gobs} \right)$ is the ego vehicle's footprint buffered by the obstacle's footprint.

\subsection{Online Optimization}
\label{subsec:online opt}

% \challen{@JL I will want feedback on the part below. I think Ram may not like it in its current form}
% During online operation, \riskmethodname{} solves an optimization problem to construct a motion plan that results in no greater than $\epsilon$ chance of collision between the ego vehicle and obstacles.
% Optimization problems with constraints such as these, which allow for some bounded level of constraint violation are called chance constrained optimizations.
% In this case, the bounded level of constraint violation is given by $\epsilon$, where $\epsilon$ is some user selected parameter for the allowable risk of the motion plan.

To construct a motion plan that ensures the ego vehicle is not-at-fault with a chance of collision at most $\epsilon$ during online planning, one could solve the following chance constrained optimization problem:
% \begin{align*}
%     \min_{p \in \P} & ~ \cost(z_0,p) \hspace{5.5cm} \opt\\
%     \text{s.t.}
%     % \begin{split} 
%     & ~ \sum_{i\in\I}\sum_{j\in\J}\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w) ~dw \leq\ \epsilon
%     % \end{split}
% \end{align*}
\begin{align*}
    \min_{p \in \P} & ~ \cost(z_0,p) \hspace{5.3cm} \opt\\
    \text{s.t.}
    % \begin{split} 
    % & ~ \new{\prob\bigg(\cup_{t\in[0,\tf]}\Big(\E\big(t,z_0,p\big) \cap \big(\cup_{i\in\I}\Oobs(t)\big) \Big)  \bigg) \leq \epsilon}\\
    % & ~ \sum_{i\in\I}\sum_{j\in\J} \prob_{i,j}\Big( \cup_{t\in T_j} \big( \E(t,z_0,p) \oplus \Gobs \big) \Big) \leq \epsilon
    &  \sum_{i\in\I}\sum_{j\in\J}\int_{ \cup_{t\in T_j} \left( \E(t,z_0,p)\oplus\zonocg{0}{\Gobs} \right)} \pdf(w) ~dw \leq \epsilon
    % \end{split}
\end{align*}
where $\cost:\Z_0\times\P \to \R$ is a user-specified cost function, and the constraint is a chance constraint that ensures the vehicle is not-at-fault with a maximum chance of collision of $\epsilon$ during the planning horizon as stated in Definition \ref{defn:notatfault-risk}.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \strikethrough{that the ego vehicle beginning from $z_0$ while tracking trajectory parameter $p$ collides with any of the obstacles over the planning horizon to be no greater than $\epsilon$.
% Because this constraint bounds the chance of violation, this problem is referred to as a chance constrained optimization problem. 
% In fact, one can establish that any solution to this optimization problem can be tracked in a not-at-fault fashion as is done in the following theorem whose proof is provided in Appendix {\ref{app: proof of thm risk cond}}:}
% % Note that if an optimal solution to \opt is found then the ego vehicle is not at fault with confidence level at least $1-\epszp - |\Inorisk|\eta$ during $[0,t_f]$ by the following theorem whose proof is provided in Appendix \ref{app: proof of thm risk cond}.
% \begin{thm}
% \label{thm: risk condition old}
%     \strikethrough{If the ego vehicle applies any feasible solution, $p^*\in\PP$, of (\texttt{Opt}) beginning from $z_0$ at $t=0$, then the ego vehicle is not-at-fault with confidence level at least $1-\epsilon$ during $[0,\tf]$.}  \Ram{what does confidence level mean...its never been defined.} \jinsun{removed}
% \end{thm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \strikethrough{To achieve risk-aware, real-time motion planning, (\texttt{Opt}) must be solved sufficiently fast, thus it is vital to efficiently evaluate the integration $\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w) ~dw$.
% Unfortunately such integration is challenging to compute in general because $\pdf$ could be an arbitrary density function satisfying Assumption {\ref{ass: obs pdf}}} \Ram{what does sufficiently mean?} \Ram{this argument would be easier to accept if you ran an experiment illustrating that just doing Monte Carlo is not fast enough}.
% \Ram{you are missing a sentence where you explain why its essential to also build something that is differentiable and why building a differentiable representation to the constraint is challenging.} \challen{Addressed}

To achieve real-time motion planning, \opt{} must be solved within $\tplan$ seconds.
Unfortunately, efficiently evaluating the chance constraint in \opt{} in a closed-form can be challenging in real applications for two reasons. 
Firstly, the exact information of the ego vehicle's location $\E(t,z_0,p)$ at any time is usually inaccessible due to the nonlinear and hybrid nature of the vehicle dynamics.
Secondly, the probability distribution that describes the uncertain observation of an obstacle's location as assumed in Assumption \ref{ass: obs pdf} can be arbitrary.
As illustrated in Section \ref{subsubsec: planning time without relaxation}, even approximating this chance constraint in a Monte-Carlo fashion is not fast enough for real-time motion planning. 
Therefore to achieve real-time performance, \riskmethodname{} seeks a closed-form approximation of the chance of collision for evaluation efficiency.
In addition, such approximation needs to be an over-approximation to ensure that \riskmethodname{} does not under-estimate the true risk of collision or generate plans that violate the not-at-fault condition from Definition \ref{defn:notatfault-risk}. 
Moreover, it is preferable that this approximation is differentiable, as providing the gradient of the constraint can speed up the solving procedure of online optimization.
We describe how we generate an approximation that satisfies these requirements in the next two sections.




% \begin{thm}
% \label{thm: risk condition}
%     Let $\{\RR_j\}_{j \in \J}$ be the set of zonotopes introduced in Theorem \ref{thm:footprint}, and let probability density function $f$ be as assumed in Assumption \ref{ass: obs pdf}.
%     Suppose the ego vehicle starts with initial condition $z_0=[(\zpos_0)^\top, (\zvel_0)^\top]^\top$ and control parameter $p$ where $\zpos_0,\zvel_0\in\R^3$, and let $\xi_j(z_0,p)$ be defined as in Theorem \ref{thm:footprint}. 
%     If
%     \begin{equation}
%         \label{eq: refine constraint}
%         \xi_j( z_0,p) \cap \zonocg{\w}{\Gobs} =\emptyset, ~ \forall j\in\J, \forall i\in\Inorisk
%     \end{equation}
%     and
%     \begin{equation}
%         \label{ineq: risk2integral} 
%         \sum_{j\in\J}\sum_{i\in\Irisk}\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} f(w) ~dw \leq\ \epszp
%     \end{equation}
%     with $\epszp$ defined in Theorem \ref{thm:threshpandz0}, then the ego vehicle is not-at-fault with confidence level at least $1-\epszp$ during $[0,t_f]$. 
% \end{thm}
% Note that the second constraint in this optimization leverages Boole's inequality to get a over-approximation of \eqref{eq: probthresh} as a set of sums and expresses the probability of collision as an integral.

% \jinsun{in my mind the chance constraint we are dealing with is:}
% \begin{equation}
% \label{eq: chance constraint}
%     \color{cyan} \prob\bigg(\Big(\cup_{t\in[0,\tf]}\E\big(z(t),z_0,p\big)\Big) \cap \big(\cup_{i\in\Irisk}\Oest_i(t)\big)\neq\emptyset \bigg) \leq \epszp
% \end{equation}
% \jinsun{Or rather, I'd like to have \eqref{eq: chance constraint} been relaxed via Boole's inequality before this subsection as:}
% \begin{equation}
%     \label{eq: chance constraint relaxed}
%     \color{cyan} \sum_{j\in\J}\sum_{i\in\Irisk}\prob\bigg(\Big(\cup_{t\in T_j}\E\big(z(t),z_0,p\big)\Big) \cap \Oest_i(t)\neq\emptyset \bigg) \leq\epszp
% \end{equation}
% \jinsun{and for notational simplicity, please define}
% \begin{equation}
%     \color{cyan} \varrho(z_0,p) := \prob\bigg(\Big(\cup_{t\in T_j}\E\big(z(t),z_0,p\big)\Big) \cap \Oest_i(t)\neq\emptyset \bigg).
% \end{equation}


% To achieve risk-aware real-time planning, chance-constrained optimization program \opt{} proposed in Section \ref{subsec:online opt} needs to be solved sufficiently fast, thus it is vital to efficiently evaluate the probability $\varrho(z_0,p \mid \Irisk)$.
% However because computing this probability in closed-form can be challenging in general, in this subsection we seek a way to generate its over-approximation that is differentiable with respect to $p$.
% We start by bounding $\varrho(z_0,p \mid \Irisk)$ from above using the integration of density function $f(w)$ for all $j\in\J$ and $i\in\Irisk$.
% Such integration is then further over-approximated in closed-form with its analytical gradient available to speed up the solving procedure of online planning.

% The following key theorem provides a way to over-estimate $\varrho(z_0,p\mid \Irisk)$ using the aforementioned FRS approximation, and gives sufficient conditions to ensure the ego vehicle being not-at-fault with some confidence level.



==> sections_long/05_reachability.tex <==
\section{Offline Reachability Analysis}
\label{sec:risk-rtd and reachability analysis}

% %%%%%%% OVERVIEW OF RISK-RTD
% % \subsection{\riskmethodname{} Overview}
% % \label{subsec:risk-rtd}

% % % To account for uncertainty without being too conservative during motion planning, we extend\riskmethodname{} allows the vehicle 
% % The proposed risk-aware motion planning framework consists of two main parts: an offline reachability analysis, and an online planning stage. 
% % In the first part, which is described in Section \ref{subsec:reachability analysis}, we first compute the reachable set of parameterized trajectories for the ego vehicle represented as a set of zonotopes.
% % The second part (Section \ref{sec:online planning}) occurs during operation of the ego vehicle online. 
% % At run-time, \riskmethodname{} begins by computing the estimated risk of serious injury to passengers should a collision occur, based on its relative velocity with respect to the obstacles in its sensor horizon.
% % When the risk of injury is at higher levels, \riskmethodname{} chooses to be conservative and finds motion plans that have a 0\% chance of collision, however, when the risk of injury is at lower levels, \riskmethodname{} can afford to be slightly less conservative and chooses motion plans that match risk levels for driving based on human driving data.
% % Once this threshold is selected the method computes a closed-form over-approximation on the probability of a collision with an obstacle given an arbitrary probability distribution estimating the obstacle location. 
% % Finally, the method performs a trajectory optimization over a set of control parameters to determine a trajectory with less than or equal to the set level of risk of crashing. 
% % % \jinsun{no discussion on real-time planning? like how planning happens while the vehicle is moving?}

% \Ram{I would probably rewrite the following two paragraphs and the lemma as an assumption. 
% The assumption states that there exists as a collection of zonotopes that contain the vehicle trajectory. 
% You also should be clear about which zonotope bounds which portion of the vehicle trajectory. 
% Then after the assumption you can reference the refine paper as to why its possible. 
% This will avoid introducing extraneous notation.
% In fact if you write this lemma well, then you can even avoid the last theorem in this section and simplify the notation throughout the paper considerably....}

% To achieve receding-horizon planning, \riskmethodname{} adopts from REFINE \cite{REFINE} the same offline reachability analysis that over-approximates parametrized vehicle behavior over $[0,\tf]$ using the Forward Reachable Set (FRS) defined as follows:
% \begin{equation}
%  \label{eq: FRS def}
% \begin{split}
%     \FRS([0,&\tf]):=\Bigg\{(x(t),y(t))\in \W\mid \exists t\in[0,\tf], p\in\P,  \\
%     &  \zvel_0 \in \Zvel_0  \text{ s.t. }\begin{bmatrix} x(t)\\ y(t) \end{bmatrix} = \pi_{xy}(z(t)), \\
%     & z \text{ is a solution of } \eqref{eq: vehicle dynamics} \text{ with } z(0) = \begin{bmatrix}
%         0_{3\times 1} \\ \zvel_0
%     \end{bmatrix}\Bigg\}
%     % & z_0 = \begin{bmatrix} \zpos_0 \\ \zvel_0\end{bmatrix}\in\Z_0 \text{ s.t. }\begin{bmatrix} x\\ y \end{bmatrix} = \pi_{xy}(z(t)), z \text{ is a}   \\
%     % & \text{ solution of } \ref{eq: dyn tilde_z} \text{ with } z(0)= \begin{bmatrix} z_0 \\  \zvel_0 \\ p \end{bmatrix} \Bigg\},
% \end{split}
%  \end{equation}
% % \subsection{Offline Reachability Analysis}
% % \label{subsec:reachability analysis}
% \noindent where $\Zvel_0\subset\R^3$ gives the initial velocity space of the ego vehicle.
% Because computing $\FRS([0,\tf])$ precisely is numerically challenging due to the nonlinearity of vehicle dynamics, \riskmethodname{} outer-approximates $\FRS([0,\tf])$ by a series of zonotopes. 
% Each of these zonotopes outer-approximate the ego vehicle's behavior over time intervals that are defined as follows.

% % \challen{I think we should add a small motivation for why we partition the FRS into smaller interval FRSs}
% % \begin{assum}
% % \label{ass: initial 0 pos condition}
% % \new{The initial condition space $\Z_0 = \{0_{3\times1}\}\times \Zvel_0$ where $\Zvel_0=\text{int}(\underline{\zvel_0}, \overline{\zvel_0})\subset\R^3$ is a 3-dimensional box representing all possible initial velocity conditions $\zvel_0$ of the ego vehicle.}
% % \end{assum}

% First, we pick a time step $\Delta_t\in\R_+$ such that $\tf/\Delta_t\in\N$, and partition time interval $[0,\tf]$ into $\tf/\Delta_t$ \emph{time segments} as $T_j=[(j-1)\Delta_t, j\Delta_t]$ for each $j\in \J=\{1,2,\ldots,\tf/\Delta_t\}$.
% By augmenting $\zvel_0$ and $p$ into $z$ as $[x(t),y(t),h(t),u(t),v(t),r(t), (\zvel_0)^\top]^\top\in\R^{9+n_p}$, one can then use the open-source toolbox CORA \cite{althoff2015introduction} to approximate $\FRS([0,\tf])$ as in the following lemma as a paraphrase of \cite[Thm. 16]{REFINE}:


% % The offline reachability analysis phase of \riskmethodname{} involves computing the \emph{Forward Reachable Set (FRS)} of the ego vehicle dynamics with parametrized control inputs using zonotopes. 
% % The zonotope FRS overapproximates all the possible behaviors of the ego vehicle over a given time horizon. 
% % \riskmethodname{} performs reachability analysis on a full-order vehicle model and leverages the controller from \cite{REFINE} can generate tight, zonotope overapproximations of the FRS of the vehicle dynamics. We compute these overapproximations because the actual FRS is difficult to compute exactly due to the hybrid nature of the system dynamics.
% % The forward reachable set of the ego vehicle can be defined as follows:
% % \begin{equation}
% %  \label{eq: FRS def}
% % \begin{split}
% %     \FRS([0,&\tf]):=\Bigg\{(x,y)\in \W\mid \exists t\in[0,\tf], p\in\P,  \\
% %     & \zvel_0\in\R^3  \text{ s.t. }\begin{bmatrix} x\\ y \end{bmatrix} = \pi_{xy}(z(t)), z \text{ is a}\\
% %     & \text{solution of } \eqref{eq: dyn tilde_z} \text{ with } z(0) = [0,0,0,(\zvel_0)^\top]^\top\Bigg\}.
% %     % & z_0 = \begin{bmatrix} \zpos_0 \\ \zvel_0\end{bmatrix}\in\Z_0 \text{ s.t. }\begin{bmatrix} x\\ y \end{bmatrix} = \pi_{xy}(z(t)), z \text{ is a}   \\
% %     % & \text{ solution of } \ref{eq: dyn tilde_z} \text{ with } z(0)= \begin{bmatrix} z_0 \\  \zvel_0 \\ p \end{bmatrix} \Bigg\},
% % \end{split}
% %  \end{equation}
% % % where $\pi_{xy}:\R^{9+n_p}\rightarrow \R^2$ is the projection operator that outputs the first two coordinates from its argument.

% % With the above definition, we introduce the following lemma which is a paraphrase of \cite[Thm. 16]{REFINE}:
% \begin{lem}
% \label{lem:FRS as zonotopes}
%     There exists a collection of zonotopes $\{\RR_j\}_{j\in\J}$ with $\RR_j\subset\R^{9+n_p}$ for all $j\in\J$ such that $\FRS([0,\tf]) \subseteq\cup_{j\in\J}\pi_{xy}(\RR_j)$.
% \end{lem}
% Note in Lemma \ref{lem:FRS as zonotopes} we have abused notation by extending the domain of  $\pi_{xy}$ to any zonotope $\Z = \zonocg{c}{G}$ in $\R^{9+n_p}$ as
% \begin{equation}
%    \pi_{xy}(\Z) = \left<\begin{bmatrix}
%     [c]_1 \\ [c]_2
%     \end{bmatrix},~\begin{bmatrix}
%     [G]_{1:} \\ [G]_{2:}
%     \end{bmatrix}\right>.
% \end{equation}
% The FRS over-approximation $\{\RR_j\}_{j\in\J}$ in Lemma \ref{lem:FRS as zonotopes} can be treated as a local representation of the ego vehicle's behavior in its body frame because $z(0)$ in \eqref{eq: FRS def} assumes zero initial condition of $[x,y,h]^\top$.
% Thus to avoid obstacles sensed in the world frame online, nonzero $[x(0),y(0),h(0)]^\top$ can be accounted for in zonotope reachable sets as shown in the following theorem.

% \begin{thm}
%     \label{thm:footprint}
% Let $\{\RR_j\}_{j \in \J}$ be the collection of zonotopes in Lemma \ref{lem:FRS as zonotopes}, and let $z$ be the solution to \eqref{eq: vehicle dynamics} with initial condition $z(0) = z_0\in\R^3\times\Zvel_0$ and control parameter $p\in\PP$.
% Then there exists a map $\xi:P(\R^{9 + n_p})\times \Z_0\times\P\rightarrow P(\W)$ such that 
% \begin{enumerate} 
%     % \item for all $j \in \J$ and $t \in T_j$, the vehicle footprint oriented and centered according to $z(t)$ is contained within $\xi(\RR_j,z_0,p)$, and
%     \item for all $j\in\J$, $\xi(\RR_j,z_0,p)$ contains the ego vehicle's footprint during $T_j$ (i.e. $\cup_{t\in T_j}\E(t,z_0,p)\subseteq \xi(\RR_j,z_0,p)$), and
%     \item $\xi(\RR_j,z_0,p)\subset\W$ is a zonotope of the form $\zonocg{c_{\xi,j}(z_0)+A_{\xi,j}\cdot p}{G_{\xi,j}}$ with some vector $c_{\xi,j}(z_0)\in\R^2$, some matrix $A_{\xi,j}\in\R^{2\times n_p}$ and some 2-row matrix $G_{\xi,j}$.
% \end{enumerate}
% \end{thm}
% \noindent The proof of Theorem \ref{thm:footprint} is provided in Appendix \ref{app: proof of thm footprint} with an explicit expression of $\xi(\RR_j,z_0,p)$ in \eqref{eq: xi def}.

% %%%%%%SLICING
% % Lastly we introduce the notion of slicing which is treated in detail in \cite[Section VI. C]{REFINE}. 
% % Slicing allows us to take a known $\zvel_0 \in \Zvel_0$ and $p \in \P$ and plug them into the computed $\{\RR_j\}_{j\in\J}$ to carve out a subset or \emph{slice} of our FRS approximation that includes the evolution of the hybrid vehicle dynamics model as it follows a parametrized trajectory given by the trajectory parameter $p$.
% % Throughout this work we shall denote these subsets or \emph{slices} of our zonotope reachable set as:
% % \begin{equation}
% % \label{eq: slice def}
% %    \hspace*{-0.2cm} \slice( \RR_j,\zvel_0,p) = \zonocg{c^\text{slc}}{[g_{\RR_j,(4 +n_p)},\ldots, g_{\RR_j,{\ell_j}}]}
% % \end{equation}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Due to the nonlinear and hybrid nature of the vehicle dynamics, it is challenging to compute the trajectory of vehicle state exactly when evaluating the chance constraint in \opt{}.
To resolve this challenge, \riskmethodname{} over-approximates the ego vehicle's trajectory using zonotopes as stated below:
\begin{assum}
\label{ass: offline reachability}
    Let $z$ be a solution to \eqref{eq: dyn tilde_z} starting from initial condition $z_0\in\Z_0$ with control parameter $p\in\PP$.
    For each $j\in\J$, there exists a map $\xi_j:\Z_0\times\PP\rightarrow P(\W)$ such that 
    \begin{enumerate}
        \item $\xi_j(z_0,p)$ contains the ego vehicle's footprint during $T_j$, i.e., $\cup_{t\in T_j} \E(t,z_0,p)\subseteq \xi_j(z_0,p)$, and
        \item $\xi_j(z_0,p)$ is a zonotope of the form $\zonocg{c_j(z_0)+A_j\cdot p}{G_j}$ with some linear function $c_j:\Z_0\rightarrow \R^2$, some matrix $A_j\in\R^{2\times n_p}$ and some 2-row matrix $G_j$.
    \end{enumerate}
\end{assum}

The collection of maps $\{\xi_j\}_{j\in\J}$ can be constructed by applying existing techniques for offline reachability analysis \cite[Section VI]{REFINE}.
In particular, $\{\xi_j\}_{j\in\J}$ can be generated by first applying the open-source toolbox CORA \cite{althoff2015introduction} to over-approximate the trajectory of the ego vehicle's state with initial condition $z_0$ and control parameter $p$ using a collection of zonotopes, where each zonotope over-approximates a segment of the trajectory during one small time interval among $\{T_j\}_{j\in\J}$, and then accounts for the ego vehicle's footprint.
The proof of Lemma 26 in \cite{REFINE} provides explicit formulas for $\xi_j$, $c_j$, $A_j$ and $G_j$.
Note formulas provided in \cite[Lemma 26]{REFINE} assumes the computation in the body frame of the ego vehicle, i.e., assuming $x(0)=y(0)=h(0)=0$.
In the case when the initial position and heading of the ego vehicle are not zeros, one can represent $\xi_j(z_0,p)$ in the world frame via frame transformation based on $z_0$.
In the remainder of this manuscript, we assume $\xi_j(z_0,p)$ is represented in the world frame. 





==> sections_long/06_implementable.tex <==
\section{An Implementable Alternative to \opt{}}
\label{sec: chance constraint}

This section describes an implementable alternative to \opt{} that can be solved rapidly.
In particular, we discuss how to relax the chance constraint in \opt{} in a conservative fashion.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Chance Constraint Relaxation}
\label{subsec:chance constraint}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.24\textwidth}
%          \includegraphics[trim={0cm, 10cm, 20cm, 0cm},clip,width=\textwidth]{figures/Relaxation.pdf}
%          \caption{PDF Integration.}
%          \label{fig: simulation result 1-riskrtd}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%          \includegraphics[trim={14cm, 10cm, 6cm, 0cm},clip,width=\textwidth]{figures/Relaxation.pdf}
%          \caption{Domain Relaxation.}
%          \label{fig: simulation result 1-riskrtd}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%          \includegraphics[trim={0cm, 1cm, 20cm, 9.8cm},clip,width=\textwidth]{figures/Relaxation.pdf}
%          \caption{Integrand Relaxation.}
%          \label{fig: simulation result 1-riskrtd}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%          \includegraphics[trim={14cm, 1cm, 6cm, 9.8cm},clip,width=\textwidth]{figures/Relaxation.pdf}
%          \caption{Closed-form Computation.}
%          \label{fig: simulation result 1-riskrtd}
%     \end{subfigure}
%     \caption{An illustration of chance constraint relaxation.
%     Given arbitrary $(i,j)\in\I\times\J$, in (a) the probability of collision between the ego vehicle and the $i$-th obstacle during time interval $T_j$ is relaxed as the integration of probability density function $\pdf(\cdot)$ over zonotope $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}\subset\W$ shown in green. 
%     In (b), $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ is over-approximated by a collection of right-angled triangles colored in white and black depending on if a triangle has nontrivial intersection with $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ or not.
%     In (c), $\pdf(\cdot)$ is approximated from below and above over each right-angled triangle using Interval Arithmetic. 
%     And in (d), the integration of the over-approximation of $\pdf(\cdot)$ over each right-angled triangle is computed in closed-form.}
%     \label{fig: chance constraint relaxation}
%     % \vspace*{-0.5cm}
% \end{figure*}
\begin{figure*}[!htb]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
         \includegraphics[trim={0cm, 18.4cm, 27.9cm, 0cm},clip,width=\textwidth]{figures/Relaxation_v4.png}
         \caption{PDF Integration (Sec \ref{subsubsec: PDF Integration}).}
         \label{fig: simulation result 1-riskrtd}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \includegraphics[trim={27.5cm, 18.4cm, 0cm, 0cm},clip,width=\textwidth]{figures/Relaxation_v4.png}
         \caption{Domain Relaxation (Sec \ref{subsubsec: Domain Relaxation}).}
         \label{fig: simulation result 1-riskrtd}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \includegraphics[trim={0cm, 0.3cm, 27.9cm, 18.5cm},clip,width=\textwidth]{figures/Relaxation_v4.png}
         \caption{Integrand Relaxation (Sec \ref{subsubsec: Integrand Relaxation}).}
         \label{fig: simulation result 1-riskrtd}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \includegraphics[trim={27.5cm, 0.2cm, 0cm, 18.5cm},clip,width=\textwidth]{figures/Relaxation_v4.png}
         \caption{Closed-form Computation (Sec \ref{subsubsec: Closed-form Computation}).}
         \label{fig: simulation result 1-riskrtd}
    \end{subfigure}
    \caption{An illustration of chance constraint relaxation.
    Given arbitrary $(i,j)\in\I\times\J$, in (a) the probability of collision between the ego vehicle and the $i$-th obstacle during time interval $T_j$ is relaxed as the integration of probability density function $\pdf$ (shown in purple and blue) over zonotope $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}\subset\W$ (shown in green). 
    In (b), $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ is over-approximated by a collection of right-angled triangles colored in white and black depending on if a triangle has nontrivial intersection with $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ or not.
    In (c), Interval Arithmetic to generate an over- and under-approximation of $\pdf$ over each right-angled triangle. 
    And in (d), the integration of the over-approximation of $\pdf$ over each right-angled triangle is computed in closed-form.}
    \label{fig: chance constraint relaxation}
    % \vspace*{-0.5cm}
\end{figure*}

The chance constraint in \opt{} is relaxed conservatively as illustrated in Figure \ref{fig: chance constraint relaxation}.
First, the risk of collision during $[0,\tf]$ is over approximated using Assumption \ref{ass: offline reachability}.
Then we relax the domain of integration into a collection of right-angled triangles and relax the PDF as a quadratic polynomial. 
Finally we describe a closed-form equation for the relaxed integral.


\subsubsection{PDF Integration}
\label{subsubsec: PDF Integration}
Recall the ego vehicle's performance during the planning horizon is over-approximated by a collection of maps $\{\xi_j\}_{j\in\J}$, then the chance constraint in \opt{} is relaxed according to the following lemma which follows directly from the first property in Assumption \ref{ass: offline reachability}:
\begin{lem}
\label{lem: risk condition}
    Suppose the ego vehicle starts with initial condition $z_0\in\Z_0$ and control parameter $p\in\PP$.
    Let the collections of probability density functions $\{\pdf\}_{(i.j)\in\I\times\J}$ and maps $\{\xi_j\}_{j\in\J}$ be as assumed in Assumptions \ref{ass: obs pdf} and \ref{ass: offline reachability}  respectively, and let matrix $\Gobs$ be as assumed in Assumption \ref{ass: swept_volume assumption}.
    For arbitrary $\epsilon\in[0,1]$, if
    \begin{equation}
    \label{ineq: pdf relaxation}
        \sum_{i\in\I}\sum_{j\in\J}\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w) ~dw \leq \epsilon
    \end{equation}
    then
    \begin{equation}
    \label{eq: chance constraint def}
    % \sum_{i\in\I}\sum_{j\in\J} \prob_{i,j}\Big( \cup_{t\in T_j} \big( \E(t,z_0,p) \oplus \Gobs \big) \Big) \leq \epsilon,
     \sum_{i\in\I}\sum_{j\in\J}\int_{ \cup_{t\in T_j} \left( \E(t,z_0,p)\oplus\zonocg{0}{\Gobs} \right)} \pdf(w) ~dw \leq \epsilon.
\end{equation}
    % \begin{equation}
    %     \stkout{\prob\bigg(\cup_{t\in[0,\tf]}\Big(\E\big(t,z_0,p\big) \cap \big(\cup_{i\in\I}\Oobs(t)\big) \Big)  \bigg) \leq \epsilon.}
    % \end{equation}
    % \begin{equation}
    %     \new{\hspace{-0.2cm}\prob\big( \{t\in[0,\tf]\mid\E(t,z_0,p)\cap\cup_{i\in\I}\Oobs(t)\}\neq\emptyset \big) \leq \epsilon. }
    % \end{equation}
\end{lem}





 
% This subsection constructs a differentiable over-approximation to the constraint in \opt{} in closed-form and computes an analytical gradient available to this expression which drastically improves performance of the online operation of \riskmethodname{}.
% To maintain conservatism while approximating the constraint in \opt{}, we relax both domain and integrand of the integration. 
% For simplicity, in the remainder of this subsection we assume that $i$ and $j$ take arbitrary values in $\I$ and $\J$, respectively. 
\subsubsection{Domain Relaxation}
\label{subsubsec: Domain Relaxation}
Recall by Assumption \ref{ass: offline reachability} that $\xi_j(z_0,p)$ can be rewritten as $\zonocg{c_{j}(z_0)+A_{j}\cdot p}{G_{j}}=\zonocg{c_{j}(z_0)}{G_{j}}+A_{j}\cdot p$.
Then to relax the domain of integration $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$, we start by constructing a $k$-by-$k$ grid that covers zonotope $\xi_j(z_0,0)\oplus\zonocg{0}{\Gobs} = \zonocg{c_{j}(z_0)}{[G_{j},\Gobs]}$ where $k$ is some user-specified positive integer.
Each cell in the grid shares the same size and is indexed by its row and column index in the grid.
Each cell in the grid is further divided into two right triangles that are indexed by 1 or -1 corresponding to the lower or upper triangles of the cell, respectively.
For convenience, denote $\T_{j,k_1,k_2,k_3}(z_0)\subset \W$ as the right triangle indexed by $k_3\in\{-1,1\}$ in the block on the $k_1$-th row and $k_2$-th column of the grid that covers $\zonocg{c_{j}(z_0)}{[G_{j},\Gobs]}$.
Define  
\begin{align}
\label{eq: bT def}
        &\hspace{-0.1cm}\bT_{j}(z_0) := \big\{\T_{j,k_1,k_2,k_3}(z_0) \mid k_1,k_2\in\{1,2,\ldots,k\}, \\
        &\hspace{0.3cm} |k_3|=1, ~ \T_{j,k_1,k_2,k_3}(z_0)\cap\zonocg{c_{j}(z_0)}{[G_{j},\Gobs]} \neq\emptyset  \big\}. \nonumber
\end{align}
% \jinsun{I used $\bT_j(z_0)$ instead of $\bT_{j,z_0}$, but with $\bT_j(z_0)$, the chance constraint of \optE{} later didn't fit in one column.}
as the collection of every possible $\T_{j,k_1,k_2,k_3}(z_0)$ that intersects with $\zonocg{c_{j}(z_0)}{[G_{j},\Gobs]}$, thus
\begin{equation}
\label{eq: zonotope covering}
 \zonocg{c_{j}(z_0)}{[G_{j},\Gobs]}\subset( \cup_{\T\in\bT_{j}(z_0)}\T).   
\end{equation}
% $\zonocg{c_{\xi,j}(z_0)}{[G_{\xi,j},\Gobs]}\subset( \cup_{\T\in\bT_j(z_0)}\T)$.
Notice $\xi_j(z_0,p) = \xi_j(z_0,0) + A_{j}\cdot p$, therefore $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs} \subset \left( (\cup_{\T\in\bT_{j}(z_0)}\T) +A_{j}\cdot p \right)$ and
\begin{align}
    \begin{split}
        \int\displaylimits_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \hspace*{-0.75cm}  \pdf(w)~dw \leq \sum_{\T\in\bT_{j}(z_0)} \int_{\T +A_{j} p}  \pdf(w)~dw. \label{ineq: int relax on region}
    \end{split}
\end{align} 
\begin{rem}
    Note that for any $\T\in\bT_{j}(z_0)$, $\T$ depends on $z_0$ and $j$. 
    However, in the interest of reducing notational complexity, we drop the dependency on $z_0$ and $j$ in the remainder of this manuscript.
    As the value of $k$ increases, one could generate a tighter cover of $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$, but processing these additional triangles may require additional computational resources.
\end{rem}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[trim=0cm 0cm 11cm 10cm, clip,width=0.7\columnwidth,clip=true]{figures/covering.pdf}
%     \caption{An illustration of covering $\zonocg{c_\xi}{[G_\xi,\Gobs]}$ in green by a grid in black with $k=9$.
%     Such 9-by-9 grid results in 64 blocks, and each block is divided into two right triangles by its diagonal in light gray. 
%     $\T_{(4,3,1)}$ and $\T_{(2,7,-1)}$ are colored in dark gray and cyan respectively. }
%     \label{fig: cover}
% \end{figure}

\subsubsection{Integrand Relaxation}
\label{subsubsec: Integrand Relaxation}

Next, we describe how to conservatively approximate the integral in the chance constraint by relaxing the integrand:
\begin{lem} \label{lem:integrandrelaxation}
 Suppose the ego vehicle starts with initial condition $z_0\in\Z_0$ and control parameter $p\in\PP$.
 Let $\T\in\bT_{j}(z_0)$ and let $\wc_\T$ denote the vertex of the right angle in $\T$.
 Define the function $\pdfT: \W \times \PP \to [0,\infty)$ as
\begin{equation}
\begin{split}
\pdfT(w,p) &:= \pdf(\wc_\T+A_{j}p)+\frac{\partial \pdf}{\partial w}(\wc_\T+A_{j}p)\cdot\\
        &\cdot(w-\wc_\T-A_{j}p)+\frac{1}{2}(w-\wc_\T-A_{j}p)^\top\cdot\\
        &\cdot H_\T\cdot(w-\wc_\T-A_{j}p),
\end{split}
\end{equation}
where $H_\T\in\R^{2\times 2}$ is generated by taking element-wise supremum of the Hessian of $\pdf$ over $\T\oplus A_{j}\PP$ using interval arithmetic \cite{hickey2001interval}.
 Then for all $w\in\T+A_{j}p$:
\begin{equation}
\label{eq: f after IA}
    \begin{split}
    \pdf(w) \leq \pdfT(w,p).
\end{split}
\end{equation}
\end{lem}
\begin{proof}
To relax the integrand $\pdf$, we start by computing the 2nd-order Taylor Expansion of $\pdf$ centered at $\wc_\T+A_{j}p$ and applying Mean Value Theorem (MVT) \cite[Theorem 4.1]{sahoo1998mean} to eliminate higher order terms in the Taylor Expansion as:
\begin{equation}
\label{eq: Taylor + MVT}
\begin{split}
    \hspace{-0.2cm}\pdf(w) = &\pdf(\wc_\T+A_{j}p)+\frac{\partial \pdf}{\partial w}(\wc_\T+A_{j}p)\cdot\\
        &\cdot(w-\wc_\T-A_{j}p)+\frac{1}{2}(w-\wc_\T-A_{j}p)^\top\cdot\\
        &\cdot\Hess_{\pdf}(w')\cdot(w-\wc_\T-A_{j}p)
\end{split}
\end{equation}
where $w'\in\T+A_{j}p$ is some point on the line segment joining points $\wc_\T+A_jp$ and $w$ in $\T+A_jp$, and $\Hess_{\pdf}$ gives the Hessian of $\pdf$.
Because MVT does not provide $w'$ in a closed-form, we then drop the dependency of $w'$ in \eqref{eq: Taylor + MVT} by bounding the Hessian of $\pdf$ as a matrix $H_\T\in\R^{2\times 2}$ where $H_\T$ is generated by taking element-wise supremum of $\Hess_{\pdf}$ over $\T\oplus A_{j}\PP$ using Interval Arithmetic \cite{hickey2001interval}.
Note by construction of $\T$ and $\wc_\T$, it is guaranteed that either $w\geq\wc_\T+A_{j}p$ for all $w\in\T+A_{j}p$ or $w\leq\wc_\T+A_{j}p$ for all $w\in\T+A_{j}p$, thus by definition of $H_\T$ the desired inequality holds for all $w\in\T+A_{j}p$.
\end{proof}

% Next we over-approximate the integration by relaxing the integrand $\pdf$.
% Given arbitrary $p\in\P$ and $\T\in\bT_{j}(z_0)$, let $\wc_\T$ denote the vertex of the right angle in $\T$, then $\wc_\T+A_{j}p$ gives the vertex of the right angle in $\T+A_{j}p$.
% To relax the integrand $\pdf$, we start by computing the 2nd-order Taylor Expansion of $\pdf$ centered at $\wc_\T+A_{j}p$ and applying Mean Value Theorem (MVT) \cite[Theorem 4.1]{sahoo1998mean} to eliminate higher order terms in the Taylor Expansion as:
% \begin{equation}
%     \begin{split}
%         f(&w) = f(\wc_\T+Ap)+\frac{\partial f}{\partial w}(\wc_\T+Ap)\cdot\\
%         &\cdot(w-\wc_\T-Ap)+\frac{1}{2}(w-\wc_\T-Ap)^\top\cdot\\
%         &\cdot\Hess_f(\wc_\T+Ap)\cdot(w-\wc_\T-Ap) + \text{H.O.T.}
%     \end{split}
% \end{equation}
% where $\Hess_f(\wc_\T+Ap)$ represents the evaluation of the Hessian of $f$ at point $\wc_\T+Ap$ given $j$ and $i$, and ``H.O.T." stands for \emph{Higher Order Terms} that converge to 0 as $w$ converges to $\wc_\T+Ap$.
% Notice $\wc_\T+Ap$ is convex in $\W\subset\R^2$, then by Mean Value Theorem \cite[Theorem 4.1]{sahoo1998mean}, for any $w\in\T+Ap$ there exists a point $w'\in\T+Ap$ on the line segment joining points $w$ and $\wc_\T$ such that 
% \begin{equation}
% \label{eq: Taylor + MVT}
% \begin{split}
%     \hspace{-0.2cm}\pdf(w) = &\pdf(\wc_\T+A_{j}p)+\frac{\partial \pdf}{\partial w}(\wc_\T+A_{j}p)\cdot\\
%         &\cdot(w-\wc_\T-A_{j}p)+\frac{1}{2}(w-\wc_\T-A_{j}p)^\top\cdot\\
%         &\cdot\Hess_{\pdf}(w')\cdot(w-\wc_\T-A_{j}p)
% \end{split}
% \end{equation}
% where $w'\in\T+A_{j}p$ is some point on the line segment joining points $\wc_\T+A_jp$ and $w$ in $\T+A_jp$, and $\Hess_{\pdf}$ gives the Hessian of $\pdf$.
% Because MVT does not provide $w'$ in a closed-form, we then drop the dependency of $w'$ in \eqref{eq: Taylor + MVT} by bounding the Hessian of $\pdf$ as a matrix $H_\T\in\R^{2\times 2}$ where $H_\T$ is generated by taking element-wise supremum of $\Hess_{\pdf}$ over $\T\oplus A_{j}\PP$ using Interval Arithmetic \cite{hickey2001interval}.
% Note by construction of $\T$ and $\wc_\T$, it is guaranteed that either $w\geq\wc_\T+A_{j}p$ for all $w\in\T+A_{j}p$ or $w\leq\wc_\T+A_{j}p$ for all $w\in\T+A_{j}p$, thus by definition of $H_\T$ the following inequality holds for all $w\in\T+A_{j}p$:
% \begin{equation}
% \label{eq: f after IA}
%     \begin{split}
%     \pdf(w) \leq &\pdf(\wc_\T+A_{j}p)+\frac{\partial \pdf}{\partial w}(\wc_\T+A_{j}p)\cdot\\
%         &\cdot(w-\wc_\T-A_{j}p)+\frac{1}{2}(w-\wc_\T-A_{j}p)^\top\cdot\\
%         &\cdot H_\T\cdot(w-\wc_\T-A_{j}p) =: \pdfT(w,p).
% \end{split}
% \end{equation}
Note the inequality in \eqref{eq: f after IA} flips if $H_\T$ is generated by taking an element-wise infimum of the Hessian of $\pdf$.
This would create under approximation to $q$.
% However because our goal is to ensure vehicle safety with a chance of collision bounded from above, an over-estimation of $q$ is preferred. 

\Ram{do we need this remark?}
\begin{rem}
    To achieve a tighter upper bound of $\pdf$ on $\T+A_{j}p$, one can replace $H_\T$ in \eqref{eq: f after IA} by some matrix $\tilde H_\T(p)\in\R^{2\times 2}$, which is computed by taking element-wise supremum of the Hessian of $\pdf$ over $\T+A_{j}p$ instead of $\T\oplus A_{j}\PP$ using interval arithmetic.
    However, recall that we aim to over approximate $\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w) ~dw$ with a closed form representation while preserving differentiability.
    Unfortunately taking the derivative of $\tilde H_\T(p)$ with respect to $p$ is challenging when using interval arithmetic.
    On the other hand, the derivative of $H_\T$ with respect to $p$ is $0$ because by construction $H_\T$ is invariant over $\PP$.
    % \new{Hence using $H_\T$ instead of $\tilde H_\T(p)$ is preferred.}
\end{rem}

\subsubsection{Closed-form Computation}
\label{subsubsec: Closed-form Computation}
As a result of \eqref{ineq: int relax on region} and \eqref{eq: f after IA}, the following inequality holds:
\begin{equation}
    \begin{split}
        &\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w)~dw\leq \\
        % &\hspace{3cm} \leq \int_{\cup_{\T\in\bT_j}\T+A_{j} p} f(w)~dw\\
        &\hspace{1.5cm} \leq \sum_{\T\in\bT_{j}(z_0)} \int_{\T +A_{j} p} \pdfT(w,p)~dw. \label{ineq: relaxed integration}
    \end{split}
\end{equation}
Notice that $\pdfT(w,p)$ defined in \eqref{eq: f after IA} is indeed a quadratic polynomial of $w$, and $\T+A_{j}p$ is a simplex in $\R^2$.
One can then compute $\int_{\T +A_{j} p} \pdfT(w,p)~dw$ in closed-form using the following theorem:

\begin{thm}
\label{thm: lasserre}
    For any $i\in\I$ , $j\in\J$, $z_0\in\Z_0$, $p\in\PP$ and $\T\in\bT_{j}(z_0)$, let $A_{j}\in\R^{2\times n_p}$ be defined as in Assumption \ref{ass: offline reachability}, let $\pdfT$ be defined as in \eqref{eq: f after IA}, and let $\idx_{k_3}(\T)$ denote the last index of its argument (i.e., $\idx_{k_3}(\T_{j,k_1,k_2,k_3}(z_0)) = k_3$).
    Assume that positive numbers $l_1$ and $l_2$ give the lengths of horizontal and vertical right angle sides of $\T$ respectively, then
    % \begin{equation}
    % \label{eq: lasserre}
    %     \begin{split}
    %         \hspace{-0.2cm}\int_{\T +A_{j} p} \pdfT(w,p)~&dw = \frac{1}{2\det(A_{\T})}\big(\fshz(p)+\\
    %         &+\fsho(p)+\fsht(p)\big) 
    %     \end{split}
    % \end{equation}
    % with
    % \begin{align}
    %     &A_\T = \begin{bmatrix}
    %             \idx_{k_3}(\T)/l_1 & 0 \\ 0 & \idx_{k_3}(\T)/l_2
    %         \end{bmatrix},\\
    %     &\hat H_\T = A_\T^{-\top} H_\T A_\T^{-1},\\
    %     &\fshz(p) = \pdf(\wc_\T+A_{j}p ), \label{eq: f0}\\
    %     &\fsho(p) = \frac{\partial \pdf}{\partial w}(\wc_\T+A_{j}p)\cdot A_\T^{-1}\cdot\begin{bmatrix}\frac{1}{3}\\\frac{1}{3}\end{bmatrix}, \label{eq: f1}\\
    %     &\fsht(p) = \begin{bmatrix}\frac{1}{4\sqrt 3} & \frac{1}{4\sqrt 3}\end{bmatrix} \left( \hat H_\T \odot \begin{bmatrix}
    %     2 & 1\\ 1 & 2
    %     \end{bmatrix}  \right)\begin{bmatrix}\frac{1}{2\sqrt 3} \\ \frac{1}{2\sqrt 3}\end{bmatrix}, \label{eq: f2}
    % \end{align}
    % where $\odot$ denotes the element-wise multiplication. 

    \begin{equation}
    \label{eq: lasserre}
    \begin{split}
        \hspace{-0.34cm}\int_{\T +A_{j} p} \pdfT&(w,p) dw =  \frac{1}{2\det(A_{\T})} \bigg( \pdf(\wc_\T+A_{j}p ) +\\
        &~+ \begin{bmatrix}\frac{1}{4\sqrt 3} & \frac{1}{4\sqrt 3}\end{bmatrix} \Big( \hat H_\T \odot \begin{bmatrix}
        2 & 1\\ 1 & 2
        \end{bmatrix}  \Big)\begin{bmatrix}\frac{1}{2\sqrt 3} \\ \frac{1}{2\sqrt 3}\end{bmatrix}+\\
        &\hspace{1.3cm}+\frac{\partial \pdf}{\partial w}(\wc_\T+A_{j}p)\cdot A_\T^{-1}\cdot\begin{bmatrix}\frac{1}{3}\\\frac{1}{3}\end{bmatrix}\bigg)
    \end{split}
    \end{equation}
    where $\odot$ denotes the element-wise multiplication and 
    \begin{align}
        &A_\T = \begin{bmatrix}
                \idx_{k_3}(\T)/l_1 & 0 \\ 0 & \idx_{k_3}(\T)/l_2
            \end{bmatrix},\\
        &\hat H_\T = A_\T^{-\top} H_\T A_\T^{-1}.
    \end{align}
\end{thm}

% This theorem follows from \cite[Theorem 1.1]{lasserre2021simple}
\begin{proof}
    The claim follows from \cite[Theorem 1.1]{lasserre2021simple} and the fact that $A_\T\big((\T+A_{j}p)-(\wc_\T+A_{j}p)\big)$ equals the canonical simplex $\Delta:= \{(x,y)\in\R^2\mid x+y\leq 1, x\geq 0, y\geq 0\}$.
\end{proof}


\subsection{Enhanced Online Optimization}
\label{subsec:enhanced online opt}
The computation in Section \ref{subsec:chance constraint} provides a tractable way to enfore not-at-fault behavior compared to the original chance constraint in \opt{}.
As a result, we solve the following optimization during online planning in \riskmethodname{}.
\begin{align*}
    \min_{p \in \P} & ~ \cost(z_0,p) \hspace{5cm} \optE\\
    \text{s.t.}
    & ~ \sum_{i\in\I}\sum_{j\in\J}\sum_{\T\in\bT_{j}(z_0)}\int_{\T +A_{j} p} \pdfT(w,p)~dw \leq\epsilon 
    % &\hspace{6.5cm}\leq\epszp
\end{align*}

\noindent\optE{} is an enhanced version of \opt{} because satisfaction of the chance constraint in \optE{} implies that satisfaction of the chance constraint in \opt{} by Lemma \ref{lem: risk condition}, \eqref{eq: zonotope covering}, and \eqref{eq: f after IA}. 
Thus the following Lemma holds based on Definition \ref{defn:notatfault-risk}.
\begin{lem}
\label{lem: feasible gives safety}
If the ego vehicle applies any feasible solution, $p^*\in \PP$, of \optE{} beginning from $z_0\in\Z_0$ at $t = 0$, then the ego vehicle is not-at-fault with a chance of collision at most $\epsilon$ during $[0,\tf]$.
% \challen{We need to bring back the proof for this Theorem again.}
\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Implementation}
% \label{sec:implementation}
% Because \optE{} is expected to be solved in real time, providing derivatives of constraints could be helpful for speeding up the solving procedure of online optimization.
% Given the implementation of set intersection constraints in \optE{} as well as their subgradients which are provided in \cite[Thm 23]{REFINE}, 
% This section provides the gradient of chance constraint in \optE{}, and explains how to evaluate the chance constraint and its gradient efficiently using parallel computation.

\subsection{Constraint Gradient and Parallelization}
\label{subsec:gradient}
To improve the speed at which we solve \optE{}, we provide derivatives of constraints to the nonlinear programming solver.
To compute the gradient of chance constraint in \optE{}, it suffices to compute the derivatives of $\int_{\T +A_{j} p} \pdfT(w,p) ~dw$ in \eqref{eq: lasserre} with respect to $p$.
Notice that $A_\T$ and $\hat H_\T$ are invariant over $\PP$, then
\begin{equation}
    \label{eq: d-lasserre}
    \begin{split}
        &\frac{\partial}{\partial p}\int_{\T +A_{j} p} \pdfT(w,p) ~dw =  \\
        &\hspace{1cm} = \frac{1}{2\det(A_{\T})}\cdot\bigg(\frac{\partial \pdf}{\partial w}(\wc_\T+A_{j}p ) \cdot A_{j} + \\
        &\hspace{1.5cm} +\begin{bmatrix}\frac{1}{3}\\\frac{1}{3}\end{bmatrix}^\top A_\T^{-\top}\Hess_{\pdf}(\wc_\T+A_{j}p)\cdot A_{j} \bigg).
    \end{split}
    \end{equation}


% To compute the gradient of chance constraint in \optE{}, it suffices to compute the derivatives of 
% % $\epszp$, 
% $\fshz(p)$, $\fsho(p)$ and $\fsht(p)$ in Theorem \ref{thm: lasserre} with respect to $p$.
% % Note the derivative of $\epszp$ is provided in Appendix \ref{app: proof of thm threshpandz0}.
% Note that since $\pdf$ is twice-differentiable as in Assumption \ref{ass: obs pdf}, then
% \begin{align}
%     &\frac{\partial \fshz}{\partial p}(p) = \frac{\partial \pdf}{\partial w}(\wc_\T+A_{j}p ) \cdot A_{j}, \label{eq: df0}\\
%     &\frac{\partial \fsho}{\partial p}(p) = \begin{bmatrix}\frac{1}{3}\\\frac{1}{3}\end{bmatrix}^\top A_\T^{-\top}\Hess_{\pdf}(\wc_\T+A_{j}p)\cdot A_{j},\label{eq: df1}\\
%     &\frac{\partial \fsht}{\partial p}(p) = \begin{bmatrix} 0 & 0 \\ 0 & 0 \end{bmatrix}.\label{eq: df2}
% \end{align}

% \subsection{Parallelization}
% \label{subsec:cuda}
Notice the computations of $\int_{\T +A_{j} p} \pdfT(w,p)~dw$ and its gradient can be parallelized for all $(i,j)\in\I\times\J$ and all $\T\in\bT_{j}(z_0)$ as indicated in Algorithm \ref{alg: cuda}.
% We summarize the parallel evaluations of the chance constraint and its gradient in \optE{} in Algorithm \ref{alg: cuda}.
$\bT_j(z_0)$ is generated in line 1 for all $j\in\J$.
The outer parallel for the loop starts at line 2 iterates every element in $\I\times\J$, and the inner parallel for loop starts at line 3 and iterates over each right-angled triangle in $\bT_{j}(z_0)$.
The integral and its gradient over each right-angled triangle are computed from lines 4 to 6.
The chance constraint and its gradient in \optE{} can be computed as the sum of all computed $\int_{\T +A_{j} p}\pdfT(w,p) ~dw$ and $\frac{\partial}{\partial p}\int_{\T +A_{j} p} \pdfT(w,p) ~dw $, respectively.

% Within the parallel for loop from line 2 to 8, $\wc_\T$ and $A_\T$ are first generated in line 3, then the over-approximation of the probability integration as well as the gradient of the over-approximation are computed in line 4-5 and line 6-7 respectively using the provided value of control parameter $p'$. 
% Finally the chance constraint and its gradient are evaluated in line 9-10.

\begin{algorithm}[t]
    \caption{Chance Constraint Parallelization}
    \label{alg: cuda}
    \begin{algorithmic}[1]
        \REQUIRE $z_0\in\Z_0$, $p\in\PP$, $\{\pdf\}_{(i,j)\in\I\times\J}$, $\{\xi_j\}_{j\in\J}$
        \STATE \textbf{Generate} $\{\bT_{j}(z_0)\}_{j\in\J}$ as in \eqref{eq: bT def} using $\{\xi_j\}_{j\in\J}$
        \STATE \textbf{Parfor} $(i,j)\in\I\times\J$ \textbf{do}
            \STATE \quad \textbf{Parfor} $\T\in \bT_{j}(z_0)$ \textbf{do}
            % \STATE \quad \textbf{generate} $\bT$ as in \eqref{eq: bT def} using $z_0$ and $\RR_j$
            \STATE \quad \quad \textbf{Compute} $\wc_\T$, $A_\T$ and $H_\T$
            \STATE \quad \quad \textbf{Compute} $\int_{\T +A_{j} p} \pdfT(w,p) ~dw $ as in \eqref{eq: lasserre}
            \STATE \quad \quad \textbf{Compute} $\frac{\partial}{\partial p}\int_{\T +A_{j} p} \pdfT(w,p) ~dw $ as in \eqref{eq: d-lasserre}
        \STATE \quad \textbf{End Parfor}
        \STATE \textbf{End Parfor}
        % \STATE \texttt{con}$\gets \sum_{i\in\I}\sum_{j\in\J}\sum_{\T\in\bT_{j}(z_0)}\int_{\T +A_{j} p} \pdfT(w,p)~dw$
        % \STATE \texttt{dcon}$\gets \sum_{i\in\I}\sum_{j\in\J}\sum_{\T\in\bT_{j}(z_0)}\frac{\partial}{\partial p}\int_{\T +A_{j} p} \pdfT(w,p)~dw$ 
        % \STATE \textbf{Accumulate} integration and the gradient over $\bT_{j}(z_0)$ and $\I\times\J$
    \end{algorithmic}
\end{algorithm}

\subsection{Online Operation}
\label{subsec: online operation}
Algorithm \ref{alg: online} summarizes the online operation of \riskmethodname{}.
It begins by sensing and constructing predictions for obstacle locations as in Assumption \ref{ass: obs pdf} (Line 1).
\texttt{OnlineOpt} then solves \optE{} to search for a not-at-fault plan with a chance of collision at most $\epsilon$ (Line 2).
If \optE{} is infeasible, then \riskmethodname{} terminates planning (Line 3), otherwise it enters the planning loop (Line 4).
Within the loop, \riskmethodname{} first resets time to 0 (Line 5) and executes the driving maneuver corresponding to $p^*$ (Line 6).
Meanwhile, \texttt{SenseObstacles} updates the predictions for obstacle locations (Line 7) and \texttt{StatePrediction} predicts the ego vehicle state at $t=\tm$ as in Assumption \ref{assum:tplan} (Line 8) to be used as the initial condition for the next planning iteration.
In the case when the predicted vehicle state $z_0\notin\Z_0$, then \riskmethodname{} breaks the planning loop (Line 9).
Otherwise \optE{} is solved again using the updated obstacle information and $z_0$ (Line 10), and \riskmethodname{} breaks the planning loop if \optE{} is infeasible or takes longer than $\tplan$ to find a solution (Line 11).
Finally once \riskmethodname{} leaves the planning loop, the contingency braking maneuver corresponding to $p^*$ is executed and \riskmethodname{} terminates planning (Line 13).
% In each planning iteration, \riskmethodname{} first checks if the provided initial condition lies in $\Z_0$.
% If $z_0\notin \Z_0$, then both the driving and contingency braking maneuvers corresponding to $p^*$ are executed and \riskmethodname{} terminates (Line 3).
% Otherwise, only the driving maneuver corresponding to $p^*$ is executed (Line 4).
% Meanwhile, \texttt{SenseObstacles} senses and predicts obstacles probabilistically as in Assumption \ref{ass: obs pdf} (Line 5).
% \optE{} is then solved to find a not-at-fault plan with a chance of collision at most $\epsilon$ (Line 6).
% If \optE{} fails to find a feasible plan within $\tplan$, the contingency braking maneuver whose safety has been verified in the last planning iteration is executed, and \riskmethodname{} terminates (Line 7).
% If a solution to \optE{} is found, \texttt{StatePrediction} predicts the ego vehicle state at $t=\tm$ as in Assumption \ref{assum:tplan} (Line 8) and uses that as the initial state $z_0$ for the next planning iteration.
% Time is also reset to 0 to prepare for the next planning iteration (Line 9).
Note, we are able to obtain the following theorem by iteratively applying Lemma \ref{lem: feasible gives safety}:


\begin{thm}
% \new{Suppose the ego vehicle can sense and predict the surrounding obstacles as in Assumption \ref{ass: obs pdf}, and starts from a not-at-fault control parameter $p_0\in\PP$ with a chance of collision at most $\epsilon$.
% Then by performing planning and execution as in Algorithm \ref{alg: online}, the ego vehicle is not-at-fault with a chance of collision at most $\epsilon$ for all time.}
Suppose the ego vehicle can sense and predict the surrounding obstacles as in Assumption \ref{ass: obs pdf}, and starts from rest with an initial condition $z_0\in\Z_0$ at $t=0$
Then by performing planning and execution as in Algorithm \ref{alg: online}, the ego vehicle is not-at-fault with a chance of collision at most $\epsilon$ for all time.
\end{thm}

\begin{algorithm}[t]
    \caption{\riskmethodname{} Online Planning}
    \label{alg: online}
    \begin{algorithmic}[1]
        \REQUIRE $z_0\in\Z_0$ and $\epsilon\in[0,1]$
        \STATE \textbf{Initialize:} $\{\pdf\}_{(i,j)\in\I\times\J}\gets\texttt{SenseObstacles}()$
        \STATE \textbf{Try} $p^*\gets\texttt{OnlineOpt}(z_0,\{\pdf\}_{(i,j)\in\I\times\J},\epsilon)$
        \STATE \textbf{Catch} terminate planning
        \STATE \textbf{Loop:} // \textit{Line 6 executes simultaneously with Line 7-11}
            \STATE \quad \textbf{Reset} $t$ to 0
            \STATE \quad \textbf{Execute} $p^*$ during $[0,\tm)$
            \STATE \quad $\{\pdf\}_{(i,j)\in\I\times\J}\gets\texttt{SenseObstacles}()$
            \STATE \quad $z_0\gets\texttt{StatePrediction}(z_0,p^*,\tm)$
            \STATE \quad \textbf{If} $z_0\notin \Z_0$, \textbf{then} break
            \STATE \quad \textbf{Try} $p^*\gets\texttt{OnlineOpt}(z_0,\{\pdf\}_{(i,j)\in\I\times\J},\epsilon)$
            \STATE \quad \textbf{Catch} break
        \STATE \textbf{End}
        \STATE \textbf{Execute} $p^*$ during $[\tm,\tf]$, \textbf{then} terminate planning
    \end{algorithmic}
\end{algorithm}


% \begin{algorithm}[t]
%     \caption{\riskmethodname{} Online Planning}
%     \label{alg: online}
%     \begin{algorithmic}[1]
%         \REQUIRE $p_0$, $z_0$ and $\epsilon$
%         \STATE \textbf{Initialize:} $p^*\gets p_0$, $t\gets 0$
%         \STATE \textbf{Loop:} // \textit{Line 4 as Line 5-8 executes simultaneously}
%             \STATE \quad \textbf{If} $z_0\notin \Z_0$, execute $p^*$ during $[0,\tf]$, then \textbf{break}
%             \STATE \quad \textbf{Execute} $p^*$ during $[0,\tm)$
%             \STATE \quad $\{\pdf\}_{(i,j)\in\I\times\J}\gets\texttt{SenseObstacles}()$
%             \STATE \quad \textbf{Try} $p^*\gets\texttt{OnlineOpt}(z_0,\{\pdf\}_{(i,j)\in\I\times\J},\epsilon)$
%             \STATE \quad \textbf{Catch} execute $p^*$ during $[\tm,\tf]$, then \textbf{break}
%             \STATE \quad $z_0\gets\texttt{StatePrediction}(z_0,p^*,\tm)$
%             \STATE \quad \textbf{Reset} $t$ to 0
%         \STATE \textbf{End}
%     \end{algorithmic}
% \end{algorithm}




% \section{Extensions: Risk Threshold Selection}
% \label{sec:risk threshold}
% % \jinsun{introduce what a chance constraint is}
% \Ram{First you have not ever defined what a chance constrained program is...so how is the reader supposed to know what $\epsilon$ means.
% Second, it seems like this subsection is in the wrong place. 
% It seems as if this is an extension to risk-rtd, where in the original risk-rtd the chance constraint is a fixed $\epsilon$.
% I'd recommend creating a seperate section right before the experimental section you describe how you can extend risk-rtd and allow for the risk threshold to vary.}
% \challen{Addressed}
% In chance-constrained motion planning problems, it is unclear how the risk threshold $\epsilon$ should be selected.
% \new{
% Most works evaluate the ego vehicle performance at different thresholds and just arbitrarily select a threshold that they deem fit and keep it constant for the entire time the robot is operating \cite{lyons_chance,wang2020,SeanFast}.}
% % Selecting the risk threshold is often a non-trivial task in chance-constrained formulations for risk aware motion planning.
% % There is the question of how exactly to select the risk threshold. 

% In this section we present a novel methodology for systematically varying the risk-threshold based on how likely it is for the passengers of the vehicle to be injured should a crash occur during the motion plan.
% \new{For the rest of this section and subsequent sections, we shall refer to this likelihood of injury should a crash occur as the risk of injury.
% This methodology allows the ego vehicle to only be conservative when it has to be to ensure passenger safety (ie. when the risk of injury is high), and be less conservative in situations where the passenger are less likely to be injured should a collision occur(ie. when the risk of injury is low).
% }

% \new{This methodology hinges on being able to compute this risk of injury at the beginning on each motion plan. to compute the risk of injury, we make the following assumption: 

% % \new{
% % \begin{assum}
% % \label{ass: ego vel}
% %     \new{There exists some upper and lower bounds of the longitudinal velocity of the ego vehicle given by $\underline{u}, \overline{u}$ such that $u(t) \in [\underline{u}, \overline{u}]$,~ for all $t \in [0, \tf]$.
% %      }
    
% % \end{assum}
% % }

% \begin{assum}
% \label{ass: obs vel}
%     \ram{I still do not understand this assumption. 
%     When you write out an assumption, its helpful if you write it in english without any abbreviations or without using mathematical symbols wherever possible like $\forall$. Again if you'll notice all preceding assumptions and definitions spell out everything like ``for all'' instead of $\forall$. 
%     Also recall that its not $i$-th vehicle its $i$-th obstacle according to the obstacle definition.}
%     \new{There exists some upper and lower bounds of the longitudinal velocity of $i$-th obstacle given by $\overline{u_{i}}$ and $\underline{u_{i}}$ such that $u_i(t) \in [\underline{u_{i}}, \overline{u_{i}}]$,~ for all $t \in [0, \tf]$.
%      }
%     \strikethrough{For the duration of the planning horizon $\tf$, $\forall i$ the longitudinal velocity of the $i$-th vehicle, $u_i(t)$ is s.t. $u_i(t) \in [\underline{u_{i}}(0), \overline{u_{i}}(0)],~ \forall t \in [0, \tf]$.}
%     \Ram{if its a bound for all $t \in [0,\tf]$ then why are you writing $[\underline{u_{i}}(0), \overline{u_{i}}(0)]$ instead of $[\underline{u_{i}}, \overline{u_{i}}]$. 
%     The way you have written it makes it seem as if the bound is only true at time $0$.} 
    
%     % $u^{est}_i(\tz) \in [\underline{u_{i}}(\tz), \overline{u_{i}}(\tz)]$ for all $i\in\I$ within its sensor horizon. $\underline{u_{i}}(\tz)$ and $ \overline{u_{i}}(\tz)$ are the lower and upper bounds for the longitudinal velocity of $\Oobs$ at $\tz$. We further assume that the obstacles move at near constant velocity over the planning horizon $\tf~ \text{s.t.}~ u_i(t) \in [\underline{u_{i}}(\tz), \overline{u_{i}}(\tz)],~ \forall t \in [0, 0+\tf]$.
    
% \end{assum}

% % where $\tz$ is set to 0, to leverage it in Section \ref{sec:risk threshold}.
% The above assumption can be satisfied by, for example, using lidar data in conjunction with an extended Kalman filter \cite{vel_EKF_zindler,almeida2013real}. 


% Additionally, we assume that the longitudinal velocity of the ego vehicle in bounded over $[0,\tnb]$.
% }


% Given the estimated velocity bounds of sensed obstacles, \riskmethodname{} then computes the relative velocity of the ego vehicle with respect to each obstacle.
% \new{
% It is important to note that the ego vehicle velocity may vary over the time interval $[0,\tnb]$ based on the planned action.
% As such, for each obstacle and ego vehicle pair, the relative velocity will vary over the time interval $[0,\tnb]$.
% Thus, to ensure that we do not underestimate the risk of injury, for each obstacle and ego vehicle pair we must compute the supremum of this range of relative velocities. }
% Let $\urel{i}$ for any $i\in\I$ be the supremum of the estimated relative velocity of the ego vehicle with respect to the $i$-th obstacle during $[0,\tnb].$ 
% We then compute the estimated risk of serious injuries (MAIS3+) \cite{MAIS3+}  to passengers should a collision occur with the $i$-th obstacle as $\injury(\urel{i})$ where $\injury:\R\rightarrow[0,1]$ gives the binary logistic model with parameters adopted from \cite[Table A]{bahouth2014benefits} \Ram{you cannot be this vague. When you cite something you need to cite a specific equation, section of the paper, etc.}. \challen{Addressed}
% For each obstacle, \riskmethodname{} then decides how conservatively this obstacle should be treated by either 1) enforcing \strikethrough{no chance of collision} \new{a near zero chance of collision} with the obstacle if the risk of serious injury is greater than some user-defined threshold $\thresh$, or 2) selecting risk levels from human crash data if it can afford to treat this obstacle less conservatively because the risk of serious injury is less than $\thresh$.

% In the first case when $\injury(\urel{i}) \geq \thresh$, precisely enforcing 0 chance of collision could be too conservative because the probabilistic description of an obstacle may have non-zero probability density for all $w\in\W$ \Ram{when you described the first case above, you wrote ``treated by either enforcing no chance of collision,'' but now you are allowing for collision?}. \challen{Addressed}
% Therefore we instead relax the chance of collision to some user-specified number $\eta>0$ sufficiently close to 0, and make the following assumption.

% % This is summarized in Lemma \ref{lem:deterministic and risk} below:

% %  \begin{defn}
% % \label{lem:deterministic and risk}
% %     For any $i \in \I$, let $\injury(\urel{i})$ be the risk of serious injury at the supremum of the relative velocity between the ego vehicle and $\Oobs(t)$. 
% %     If $\injury(\urel{i}) < \thresh$, then let $i \in \Irisk$, else $i \in \Inorisk$. 
% % \end{defn}
% % For the $i$-th obstacle with $i \in \Inorisk$, we enforce that our ego vehicle cannot intersect at all with the zonotope that overapproximates the uncertain region buffered by the obstacle footprint first introduced in Assumption \ref{ass: obs pdf}.
 
% \begin{assum}
% \label{ass: uncertainty_overapp}
%     % Let $\Govr$ be a 2-row matrix s.t. $\zonocg{\w}{\Govr}\subset\W$ over-approximates the uncertain region given by $f(\w)$ that has a non-trivial probability density.

%     For each $(i,j)\in\J\times\I$, there exists a 2-row matrix $\Govr$ such that \Ram{does this $G^\text{ovr}_{i,j}$ depend on $\eta$?} \challen{Addressed, but @Ram we are not satisfied with this notation for $\Govr$, but we don't have better options for now. We wanted to know if you had any ideas for cleaner notation for $\Govr$}
%     % $f(\w)\geq\eta$ for all $\w\in\zonocg{\mathbb{E}_f(w)}{\Govr}\subset\W$, 
%     \begin{equation}
%         1-\int_{\zonocg{\mathbb{E}_\pdf(w)}{\Govr}}\pdf(w)dw\leq\eta
%     \end{equation}
%      where $\mathbb{E}_\pdf(w)$ is the expectation of the location of the $i$-th obstacle over $T_j$ satisfying $\pdf$. 
% \end{assum}

% Based on Assumption \ref{ass: uncertainty_overapp}, zonotope $\zonocg{\mathbb{E}_\pdf(w)}{\Govr}$ captures almost all probability mass of $\pdf$ given $(i,j)\in\I\times\J$.
% \Ram{I believe this sentence either has a typo or I am fundamentally not understanding the logic. In particular I believe the first clause should be $\xi\big(\RR_j,z_0,p\big)  \cap \zonocg{\mathbb{E}_f(w)}{\Govr} = \emptyset$} \challen{Addressed}
% Therefore $\xi_j(z_0,p)  \cap \zonocg{\mathbb{E}_\pdf(w)}{\Govr} = \emptyset$ implies that $\prob\Big(\big(\cup_{t\in T_j}\E(t,z_0,p)\big)\cap\big(\cup_{t\in T_j}\OO_i(t)\big) \neq\emptyset\Big) \leq\eta$.
% For notational simplicity, define $\Inorisk:=\{i\in\I\mid \injury(\urel{i}) \geq \thresh\}$ and $\Irisk:=\{i\in\I\mid \injury(\urel{i}) < \thresh\}$.

% % This is given by the first constraint in the optimization in \ref{subsec:online opt}.
% % \begin{equation}
% %     \quad \E\big(z(t),z_0,p\big)  \cap \zonocg{\w}{\Gobs} \neq \emptyset
% % \end{equation}
% For the $i$-th obstacle with $i \in \Irisk$ we apply our chance constraint from \optE{} and set the risk threshold to match human risk levels. 
% We estimate human risk levels based on the percentage of licensed drivers that are involved in crashes per year using crash statistics from the National Highway Traffic Safety Agency (NHTSA) \cite{NHTSA2019}. 
% We leverage the crash data reported at various driving speeds to get a set of human risk data that varies as a function of traveling velocity. 
% The following polynomial $\dyneps: \R \to  \R$ was used to fit these data with an $R$-squared value of 0.965 to obtain a closed-form approximation of these human risk levels: 
% \begin{equation}
%     \begin{split}
%      &\dyneps(u(t)) = 1.53\times10^{-8}u^4(t) - 1.84\times10^{-6}u^3(t)\\ 
%      & + 5.49\times10^{-5}u^2(t)+ 1.1\times10^{-4}u(t) + 2.23\times10^{-5}
%      \end{split}
%      \label{eq: def dyneps}
% \end{equation}
% where $u(t)$ is in miles per hour (mph). 
% $\dyneps$ is a continuous function that gives the risk levels human drivers use as as function of their traveling velocity.
% Recall that  $[0, \tnb]$ is the time interval that the driving maneuver is executed in. 
% Depending on the driving maneuver, $u(t)$ will vary over $t \in [0, \tnb]$. 
% To ensure that we do not exceed human risk levels over the execution of the trajectory we select a lowest human risk threshold, i.e. $\inf_{t\in[0,\tnb]}\dyneps(u(t))$,  over our range of velocities during the trajectory. 
% % Specifically, we select a threshold that corresponds to $\inf_{t\in[0,\tnb]}\big(\dyneps(u(t))\big)$. 
% % The following theorem allows us to express our $\dyneps(u(t))$ with respect to $z_0$ and $p$, so that the derivative of $\dyneps(u(t))$ can be provided to speed up the solving procedure of online planning.
% The following theorem shows that  $\inf_{t\in[0,\tnb]}\dyneps(u(t))$ is piece-wise differentiable, which can be helpful to increase the solving procedure of online optimization as presented in the next subsection. 

% % Let $u^{des}(t)$ be the desired longitudinal velocity of the ego vehicle.

% \begin{thm}
%     \label{thm:threshpandz0}
% Let $u$ be the longitudinal velocity of the solution to \eqref{eq: dyn tilde_z} from initial condition $z_0\in\Z_0$ \strikethrough{propagating with} \new{with control parameter} $p\in\PP$ \Ram{you keep using the word propagate, but never define what it means. I removed it from the place where you defined it earlier, but i'll let you remove it from here.}.
% There exists some piece-wise differentiable function $\epsilon: \Z_0\times\PP\rightarrow[0,+\infty)$ such that $\epszp=\inf_{t\in[0,\tnb]}\dyneps(u(t))$.
% \end{thm}
% \begin{proof}
%     See Appendix \ref{app: proof of thm threshpandz0}.
% \end{proof}
% Note that in Theorem \ref{thm:threshpandz0} we have abused notation and have allowed $\epsilon$ to vary as a function of $z_0$ and $p$. 

% % Leveraging the above theorem we can formulate our chance constraint as shown below:
% % \begin{equation}
% %     \label{eq: probthresh}
% %     \begin{split}
% %      &\prob\bigg(\cup_{t\in[0,\tf]}\Big(\E\big(z(t),z_0,p\big)\cap \big(\cup_{i\in\Irisk}\Oest_i(t)\big)\neq\emptyset \Big)\bigg)\\ 
% %      & \hspace{5.5cm}\leq \epszp \\
% %      \end{split}
% % \end{equation}
% % where $\epszp$ is dynamically chosen at the beginning of each maneuver as described earlier in this section.
% \new{
% This varying threshold allows us to dynamically select the risk threshold based on the risk of injury to the passenger beginning of each planning iteration, instead of arbitrarily setting a constant $\epsilon$ value as done in the earlier chance constraint in \optE.}
% \new{
% With this varying threshold we instead solve the following optimization: 
% }
% \new{
% \begin{align*}
%     \min_{p \in \P} & ~ \cost(z_0,p) \hspace{5cm} \optCV\\
%     \text{s.t.}
%     & ~ \xi\big(\RR_j,z_0,p\big)  \cap \zonocg{\mathbb{E}_{\pdf}(w)}{\Govr} \neq \emptyset, \\
%     & \hspace{5.3cm} \forall i \in \Inorisk, j\in\J\\
%     & ~ \sum_{i\in\Irisk}\sum_{j\in\J}\sum_{\T\in\bT_{j}(z_0)}\int_{\T +A_{j} p} \pdfT(w,p)~dw \leq\epszp 
%     % &\hspace{6.5cm}\leq\epszp
% \end{align*}
% }
% where $\cost: \Z_0\times\P \to \R$ is a user-specified cost function. 
% \new{The first constraint conservatively bounds the uncertain region with a zonotope and ensures that any solution found by \riskmethodname{} has a near-zero chance of colliding with all $\Oobs$ such that $i \in \Inorisk$.
% The second constraint is similar to the chance constraint introduced in \optE{}, except that $\epszp$ has replaced $\epsilon$ and it only accounts for all $\Oobs$ such that $i \in \Irisk$.
% The not-at-fault behavior of the vehicle is given by the following theorem whose proof is provided in Appendix \ref{app: proof of thm risk cond updated}.
% }
% % Note that if an optimal solution to \opt is found then the ego vehicle is not at fault with confidence level at least $1-\epszp - |\Inorisk|\eta$ during $[0,t_f]$ by the following theorem whose proof is provided in Appendix \ref{app: proof of thm risk cond}.
% \begin{thm}
% \label{thm: risk condition updated}
%     If the ego vehicle applies any feasible solution, $p^*\in\PP$, of \optCV ~beginning from $z_0$ at $t=0$, then the ego vehicle is not-at-fault with a chance of collision at most $\epsilon(z_0,p^*)+|\Inorisk||\J|\eta$ during $[0,\tf]$. 
% \end{thm}


==> sections_long/07_experiments.tex <==
\section{Experiments and Results}
\label{sec:experiments}

This section describes the application of \riskmethodname{} in simulation and on hardware using a $\frac{1}{10}$th-scale All-Wheel-Drive car-like robot, Rover, based on a Traxxas RC platform. 
We first verify the tightness and computational efficiency of proposed over-approximation of the chance integration $\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w)~dw$ as in Section \ref{subsec:chance constraint}.
Next we test the proposed \riskmethodname{} framework in simulation.
We then investigate the components that contribute to \riskmethodname{}'s performance using an ablation study.
Lastly, we demonstrate \riskmethodname{} running in real-time on a hardware platform.
All experiments are conducted in MATLAB R2021b on a laptop with an 8 Cores Intel i9-10980HK CPU, an Nvidia GeForce RTX 3080 GPU, and 32GB RAM. 
Parallelization is performed on the GPU using CUDA 11.0.
We solve our online optimizations in both simulation and on the hardware platform using IPOPT.

\subsection{Evaluation on Tightness and Computational Efficiency}
For effective motion planning, we desire a tight over-approximation to the risk of collision.
To evaluate the tightness of our over-approximation, we compare the proposed method of chance integration approximation against Monte-Carlo integration \cite[Chapter 4]{caflisch1998monte}, the Cantelli inequality \cite[Section IV B]{wang2020}, and the Chance-Constrained Parallel Bernstein Algorithm (CCPBA) \cite[Chapter 6]{SeanFast} on 3039 randomly generated tests \Ram{why choose a non-round number...}.
In each test, $(i,j,z_0,p)$ is randomly chosen from $\I\times\J\times\Z_0\times\PP$, $\xi_j$ is randomly chosen from the zonotope reachable sets for the vehicle, and $\pdf$ is set to be the probability density function of a 2-dimensional (2D) Gaussian distribution with randomly generated mean and variance. 
% Moreover, $\zonocg{0}{\Gobs}$ is set to be $\Oego\oplus\Int([0,0]^\top,[\vegomax\cdot\Delta t,0]^\top)$ in which we assume that footprints of all other vehicles on the road share the same size as the footprint of the ego vehicle, all other vehicles have zero headings, and all other vehicles travel with speeds no greater than $\vegomax$ during any time interval of length $\Delta t$.  
When apply the proposed method, the integration area $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ is covered by a 24-by-24 grid to generate $\bT_j(z_0)$. 

We treat the Monte-Carlo integration of $\pdf$ over $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ as the ground truth value of $\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w)~dw$.
This Monte-Carlo integration is performed by randomly sampling the world space $10^6$ times according to $\pdf$ and counting the number of samples that fall inside $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$.
% and integration $\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} f(w)~dw$ is bounded from above by $\rho(p)$ via Algorithm \ref{alg: CPU}.
Because CCPBA can only integrate over a polynomial set, to utilize CCPBA we approximate $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ as the superlevel set of some polynomial using polynomial optimization.
We also point out that such approximation has to be conservative to provide an upper bound of $\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w)~dw$.
% We also compare the proposed method against the upper bound of  $\int_{\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}} \pdf(w)~dw$ computed using Cantelli's inequality. 
% Another reason of why we make the polynomial approximation larger than $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ is that polynomial reachable sets are in general more conservative than zonotope reachable sets.

As shown in Figure \ref{fig: risk vs sos vs monte-carlo}, compared to CCPBA and the Cantelli inequality, the proposed method provides significantly tighter upper bounds to the ground truth on all 3039 random tests.
This is because CCPBA has to integrate over a larger area than the proposed method, and the Cantelli inequality must be valid for all probability density functions that share the same moments.
The risk approximation error, which is the difference between the Monte-Carlo integration and each method's upper bound of the risk of collision, is illustrated in Table \ref{table: integration on Gaussian} along with the associated average and maximum times to compute the upper bound.
The results from Table \ref{table: integration on Gaussian} show that \riskmethodname{} is about 60\% faster than CCPBA, but not as fast as evaluating the Cantelli inequality.

\begin{figure}[!tb]
    \centering
    \includegraphics[width=1\columnwidth]{figures/probability_error.pdf}
    \caption{This figure illustrates the results for the risk of collision estimation error for Cantelli, CCPBA, and \riskmethodname{}. 
    Note that Monte-Carlo integration with $10^6$ samples is treated as the ground truth risk of collision.
    \riskmethodname{} is able to get a risk estimation error that is an order of magnitude lower than CCPBA and the Cantelli Inequality.
    \challen{Will be moved to the Appendix, kept here for now for the sake of completeness for your read through @ramv}}
    \label{fig: risk vs sos vs monte-carlo}
\end{figure}

\begin{table}[!tb]
    \centering
    \begin{tabular}{|c||c|c|}
    \hline 
    \multirow{2}{*}{\textbf{Method}} & \textbf{Error} & \textbf{Solve Time [ms]} \\
     & \textbf{(Mean, Max)} & \textbf{(Mean, Max)}\\\hline
      Cantelli & (0.1774, 0.3420) & \textbf{(0.0181, 2.5223)}\\\hline
    CCPBA & (0.1881, 0.2149) & (1.1012, 3.5820)\\\hline
    \riskmethodname{} & \textbf{(0.0073, 0.0523)} & (0.4372, 2.3150) \\\hline
    \end{tabular}
    \caption{The results for the probability of collision estimation error of \riskmethodname{}, CCPBA, and the Cantelli Inequality when the obstacle uncertainty is represented as a Gaussian distribution. \jinsun{first row inconsistent}}
    \label{table: integration on Gaussian}
\end{table}


% \begin{table}[!tb]
%     \centering
%     \begin{tabular}{|c||c|c|c|c|}
%     \hline 
%     \multirow{2}{*}{\textbf{Method}} & \textbf{Average} & \textbf{Max.} & \textbf{Average} & \textbf{Max.} \\
%      & \textbf{Error} & \textbf{Error} & \textbf{Runtime [ms] }& \textbf{RunTime [ms]} \\\hline
%       Cantelli & 0.1774 & 0.3420 & \textbf{0.0181} & 2.5223\\\hline
%     CCPBA & 0.1881 & 0.2149 & 1.1012 & 3.5820\\\hline
%     \riskmethodname{} & \textbf{0.0073} & \textbf{0.0523} & 0.4372 & \textbf{2.3150} \\\hline
%     \end{tabular}
%     \caption{The results for the probability of collision estimation error of \riskmethodname{}, CCPBA, and the Cantelli Inequality when the obstacle uncertainty is represented as a Gaussian distribution. \jinsun{first row inconsistent}}
%     \label{table: integration on Gaussian}
% \end{table}

To test the ability of the proposed method to generalize to other probability distributions, we reuse the aforementioned 3039 random tests.
However, in this experiment the $\pdf$ is set to be the probability density of either a randomly generated bivariate beta distribution \cite{olkin2015constructions} or a multimodal distribution as a mixture of two randomly generated 2D Gaussian distributions. 
The ground truth of the probability density integration is also generated using Monte-Carlo integration in the same fashion as earlier.
Because CCPBA is unable to handle a distribution that is not Gaussian, we only evaluate \riskmethodname{} and the Cantelli inequality on these probability distributions.
As shown in Table \ref{table: integration on exponential family}, the proposed method is able to consistently provide tight over-approximations of the risk of collision when $\pdf$ describes a Gaussian distribution, a 2D beta distribution, or a multimodal distribution. 


\begin{table}[!tb]
    \centering
    \begin{tabular}{|c||c|c|c|}
    \hline 
    \multirow{2}{*}{\textbf{Method}} & \textbf{Gaussian Error} & \textbf{2D Beta Error}  & \textbf{Multimodal Error} \\
     & \textbf{(Mean, Max.)} & \textbf{(Mean, Max.)} & \textbf{(Mean, Max.)}  \\ \hline
    \riskmethodname{} & \textbf{(0.0073, 0.0523)} & \textbf{(0.0065, 0.0489)} & \textbf{(0.0079, 0.0262)} \\ \hline
    Cantelli &  (0.1774, 0.3420) & (0.2221, 0.5062) & (0.4734, 0.5851)\\ \hline
    \end{tabular}
    \caption{Results for the probability of collision estimation error of \riskmethodname{} and the Cantelli Inequality when the obstacle location is represented by probability distributions from the exponential family.
    }
    \label{table: integration on exponential family}
\end{table}


\subsection{Simulations}
\label{subsec:sim}

We compare \riskmethodname{} to two state-of-the-art chance-constrained motion planning algorithms: CCPBA \cite{SeanFast} and Cantelli MPC \cite{wang2020} and one state-of-the-art deterministic motion planning algorithm REFINE \cite{REFINE} in a realistic driving scenario.
Additionally, we evaluate how varying the risk threshold ($\epsilon$) for \riskmethodname{} affects the ego vehicle behavior in unprotected left turn scenarios.
The desired trajectory as in Definition \ref{def:traj_param} is adapted from \cite[Sec. IX-A]{REFINE} to achieve maneuvers of speed change, direction change, and lane change.
\Ram{what model parameters are you using? You claim its an F1 at the beginning of the simulation section, but I think you are using a highway model here...}

\subsubsection{Single Planning Horizon 3 Lane Highway Environment}
\challen{This section we anticipate will go to the Appendix. Keeping it here for now for your read through @ramv. If you agree we will move over the relevant experimental setup stuff covered here to the Multiplanning experiment section.}
\label{subsec: single_plan_sim}

This experiment compares the performance of \riskmethodname{} to CCPBA, Cantelli MPC, and REFINE in a 3 lane highway driving scenario in simulation over 10 randomly generated scenarios. 
Each scenario contains 1 static obstacle and between 4 to 9 dynamic obstacles, where the number of dynamic obstacles was randomly selected for each scenario.  
The initial speed of all dynamic obstacles are also randomly sampled from between 15[m/s] to 20[m/s] each scenario.
In each of these scenarios, a full-size FWD vehicle as the ego vehicle is randomly initialized in a lane, and is commanded to get as close as possible to a given waypoint in a different lane in a single planning iteration, with constant risk threshold $\epsilon = 0.05$ and $\tplan = 3$[sec].
Specification of the full-size FWD vehicle used in this work can be found in \cite[Section IX B.] {REFINE}, from which we adapt the vehicle controller and zonotope reachable sets as well.
Each scenario is simulated for 200 trials, resulting in a total of 2000 simulation cases.

Among the 200 trials of the same scenario, for arbitrary $(i,j)\in\I\times\J$, the $i$-th obstacle is always initialized with the same state, but follows different trajectories each trial. 
% These trajectories however satisfy the same probability density function $\pdf$ during $T_j$ where $\pdf$ is randomly generated for each scenario.
These trajectories are selected such that the locations of the $i$-th obstacle at the middle time of $T_j$ are randomly sampled from $\pdf$ for each trial, where $\pdf$ is kept constant for all trials of the same scenario for any $(i,j)\in\I\times\J$ \Ram{Are we still doing this given the updates on the definitions from above?}. 
To ensure that we can compare to CCPBA, we choose the $\pdf$ describing each obstacles location as a Gaussian.
For each $i\in\I$, $\pdf$ is constructed such that its mean is at the center of a lane with constant speed as $j$ increases within $\J$ \Ram{I don't understand what the latter portion of this sentence means. What does ``as  $j$ increases within $\J$ have to do with constant speed....}.
% The uncertain observation of each dynamic obstacle at any time is described by a Gaussian distribution centered along the trajectory that the dynamic obstacle would follow, assuming it started in the middle of a given lane, and maintained a constant velocity and constant heading parallel to the lane.
% The uncertain observation of each moving vehicle at any time $t_g \in [0,T_g]$ where $T_g$ is the time that the ego vehicle reaches the 1000[m] goal is described by a Gaussian distribution centered at $\begin{bmatrix}x_i(0) + u_i(0)*t_g\\\ y_0\end{bmatrix}$. $x_i(0)$, $y_i(0)$ are initial $x$ and $y$ coordinates in the global frame of the $i$-th obstacle at $t_g=0$ and $u_i(0)$ is the initial longitudinal velocity of the $i$-th obstacle at $t_g=0$. \challen{We haven't defined global frame yet, so this sentence above needs to be work-shopped.}
Recall, from Definition \ref{def: footprint}, that $L$ and $W$ are the length and width of each obstacle, respectively.
For any $(i,j)\in\I\times\J$, the standard deviation $\sigma_{i,j}$ of $\pdf$ is chosen such that the $3\sigma_{i,j}$-region of the Gaussian distribution covers the area of width $3.7-W$ and length $L+u_i(0)\cdot \Delta_t$, where $u_{i}(0)$ is the speed of the $i$-th obstacle at time 0.
Note the choice of width $3.7-W$ ensures that the footprint of the obstacle always stays inside the lane. 

% REFINE, on the other hand, is a deterministic motion planning algorithm.
Because REFINE is a deterministic motion planning algorithm, it assumes perfect knowledge of the locations of obstacles.
In scenarios where there is uncertainty in the location of obstacles, deterministic algorithms like REFINE often generate motion plans to avoid the entire uncertain region.
However, because Gaussian distributions have non-trivial probability density over the entire space $\W$, applying REFINE naively would require avoiding the entire space.
As such, we require that REFINE avoid a box that over approximates the 5-$\sigma_{i,j}$ region of the Gaussian distribution for any $(i,j)\in\I\times\J$ as shown in Figure \ref{fig: simulation result 1-refine}.
Note such 5-$\sigma_{i,j}$ region accounts for 99.99999\% of the probability mass.
% This 5-$\sigma$ region accounts for 99.99999\% of the probability mass

Table \ref{table: singleplan highway result} summarizes \riskmethodname{}, CCPBA, Cantelli MPC, and REFINE's performance on the 3 lane single planning horizon scenarios.
\riskmethodname{} was able to successfully execute the lane change maneuver 81.8\% of the time, and the other 18.2\% of the time it either decided to stay in lane, or was unable to find a solution so executed its fail-safe stopping maneuver.
It did not have any crashes in these 2000 trials.
CCPBA was able to successfully execute the lane change maneuver 55.2\% of the time,  either stayed in lane or came to a safe stop 44.8\% of the time. 
It also did not have any crashes.
Cantelli MPC was only able to successfully execute the lane change maneuver 9.1\% of the time, either stayed in lane or came to a safe stop 55.5\% of the time and crashed 35.4\% of the time.
\Ram{need a sentence about refine here.}
\riskmethodname{} was able to achieve a higher success rate than CCPBA and Cantelli MPC due to the fact that it is able to more closely approximate the ground truth risk of collision as shown in Table \ref{table: integration on Gaussian}.
This allows \riskmethodname{} to generate plans that navigate the ego vehicle through more difficult scenarios, while conservative over approximation of the risk of collision is likely to yield plans that are infeasible \Ram{this will need to be updated once REFINE results are in.}.
Cantelli MPC had a relatively substantial number of crashes, because unlike \riskmethodname{} and CCPBA, Cantelli MPC does not have a fail-safe maneuver for when it cannot find a solution.
As a result, when Cantelli MPC cannot find a solution it just continues executing its previous action, where it just maintains it velocity within its lane while it searches for a new solution.
% In some scenarios where there was an obstacle in front of it in its current lane, maintaining velocity resulted in these crashes. 

Figure \ref{fig: single planning iteration} illustrates an example case in which the chance of collision is limited by $5\%$.
In this case because Cantelli MPC fails to find a feasible plan, the ego vehicle ends up crashing into the vehicle in front of it. 
Note both \riskmethodname{} and CCPBA had 0 crashes for these 2000 trials due to the fact that they still over-approximate the risk of collision.
In the plans that they are able to execute, the actual probability of crashing evaluated via Monte-Carlo integration is usually around 0.1\%, which is much smaller than $5\%$, so it is possible to see no crash within just 2000 trials \Ram{I don't understand this last sentence.}.
\challen{An appendix with the detailed analysis of the conservatism will be added}


% \challen{Figure \ref{fig: single planning iteration} will be regenerated}
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.5\textwidth}
%          \includegraphics[trim={0cm, 6cm, 0cm, 0cm},clip,width=\textwidth]{figures/Risk_case1.pdf}
%          \caption{\riskmethodname{} utilized.}
%          \label{fig: simulation result 1-riskrtd}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.5\textwidth}
%          \includegraphics[trim={0cm, 6cm, 0cm, -0.5cm},clip,width=\textwidth]{figures/CCPBA_case1.pdf}
%          \caption{CCPBA utilized.}
%          \label{fig: simulation result 1-CCPBA}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.5\textwidth}
%          \includegraphics[trim={0cm, 6cm, 0cm, -0.5cm},clip,width=\textwidth]{figures/cantelli_case1.pdf}
%          \caption{Cantelli MPC utilized.}
%          \label{fig: simulation result 1-cantelli}
%      \end{subfigure}
%     \caption{Example of a simulated scenario in which \riskmethodname{} and CCPBA are able to navigate the ego vehicle (black) to the provided waypoint (black cross) through a lane change maneuver solved by one planning iteration, while Cantelli MPC results in a crash.
%     Forward reachable sets are shown in green.
%     Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
%     Probability distributions are illustrated as colored ellipses where the probability density from low to high are illustrated from blue to yellow.
%     Note that for visualization purposes we have buffered the probability distributions shown in this figure by the footprints of the obstacles}
%     \label{fig: single planning iteration}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.489\textwidth}
%          \includegraphics[trim={0cm, 7.8cm, 6.6cm, 0cm},clip,width=\textwidth]{figures/merge_risk.pdf}
%          \caption{\riskmethodname{} utilized.}
%          \label{fig: simulation result 1-riskrtd}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.489\textwidth}
%          \includegraphics[trim={0cm, 7.8cm, 6.6cm, -0.5cm},clip,width=\textwidth]{figures/merge_ccpba.pdf}
%          \caption{CCPBA utilized.}
%          \label{fig: simulation result 1-CCPBA}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.489\textwidth}
%          \includegraphics[trim={0cm, 7.8cm, 6.6cm, -0.5cm},clip,width=\textwidth]{figures/merge_cantelli.pdf}
%          \caption{Cantelli MPC utilized.}
%          \label{fig: simulation result 1-cantelli}
%      \end{subfigure}
%     \caption{Example of a simulated scenario in which \riskmethodname{} and CCPBA are able to navigate the ego vehicle (black) to the provided waypoint (black cross) through a lane change maneuver solved by one planning iteration, while Cantelli MPC results in a crash.
%     Forward reachable sets are shown in green.
%     Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
%     Probability distributions are illustrated as colored ellipses where the probability density from low to high are illustrated from blue to yellow.
%     Note that for visualization purposes we have buffered the probability distributions shown in this figure by the footprints of the obstacles}
%     \label{fig: single planning iteration}
% \end{figure}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[trim={0cm, 9.15cm, 8.4cm, 0cm},clip,width=\textwidth]{figures/merge_risk_v4.pdf}
         \caption{\riskmethodname{} utilized.}
         \label{fig: simulation result 1-riskrtd}
     \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[trim={0cm, 9.15cm, 8.4cm, 0cm},clip,width=\textwidth]{figures/merge_ccpba_v4.pdf}
         \caption{CCPBA utilized.}
         \label{fig: simulation result 1-CCPBA}
     \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[trim={0cm, 9.15cm, 8.4cm, 0cm},clip,width=\textwidth]{figures/merge_cantelli_v4.pdf}
         \caption{Cantelli MPC utilized.}
         \label{fig: simulation result 1-cantelli}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\textwidth}
         \includegraphics[trim={0cm, 9.15cm, 8.4cm, 0cm},clip,width=\textwidth]{figures/merge_refine_v4.pdf}
         \caption{REFINE utilized.}
         \label{fig: simulation result 1-refine}
     \end{subfigure}
    \caption{Example of a single iteration of a simulated scenario in which \riskmethodname{} is able to navigate the ego vehicle (black) to the provided waypoint (black cross) through a lane change maneuver solved by one planning iteration, while CCPBA and REFINE execute braking maneuvers as they are unable to find feasible solutions.
    Cantelli MPC results in a crash, as it has no fail-safe stopping maneuver so it instead maintains its velocity and continues searching for a feasible solution to execute the lane change.
    Forward reachable sets are shown in green.
    Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
    Probability distributions are illustrated as purple and blue ellipses where the probability density from low to high is illustrated from blue to purple.
    Note that for visualization purposes we have buffered the probability distributions shown in this figure by the footprints of the obstacles.
    Lastly, the the convex hull that REFINE uses to over-approximate the 5-$\sigma$ regions of the obstacle probability distributions are shown as gray boxes around the obstacles.
    Note that the distances on the x-axis and y-axis are in [m].}
    \label{fig: single planning iteration}
\end{figure*}

\begin{table}[!tb]
    \centering
    \begin{tabular}{|c||c|c|c|c|}
    \hline 
    \multirow{2}{*}{\textbf{Method}} & \textbf{Success} & \textbf{Crash} & \textbf{Other} & \textbf{Mean} \\ 
    & \textbf{[\%]} & \textbf{[\%]} & \textbf{Action [\%]}  & \textbf{Solve Time}\\\hline
    \riskmethodname{} & \textbf{81.8} & \textbf{0.00} & \textbf{18.2} & 0.412 $\pm$ 0.271 \\\hline
    CCPBA & 55.2 & \textbf{0.00} & 44.8 &  \textbf{0.291 $\pm$ 0.124}  \\ \hline
    Cantelli MPC & 9.10 & 35.4 & 55.5 & 0.643 $\pm$ 0.141 \\\hline
    REFINE & TBA & TBA & TBA & 0.341 $\pm$ 0.113 \\\hline
    
    % \methodname & 27\% & 0\% & 73\% & 16.5927[m/s] &  (0.2537[s], 1.3042[s])  \\ \hline
    \end{tabular}
    \caption{Single planning iteration results using \riskmethodname{}, CCPBA and Cantelli MPC. ``Other Action" encompasses the trials where each method did not complete the lane change maneuver, but instead either executed a safe stop maneuver or decided to keep driving in lane. }
    % \challen{I did sig figs since with matching decimal places the difference in number alignment was visually unappealing.}}
    
    \label{table: singleplan highway result}
\end{table}

\subsubsection{Multiple Planning Horizon 3 Lane Highway Environment}
\label{subsec: multiple_plan_sim}

This experiment evaluates how executing multiple planning iterations in succession, as is required in real-life highway settings, affects the success and crash rates of \riskmethodname{} in comparison to CCPBA, Cantelli MPC and REFINE.
We compare the methods over a 1000 randomly generated 3-lane highway scenarios in simulation with a constant $\epsilon$ value set to 0.05.
In each simulation scenario the ego vehicle is expected to navigate through dynamic traffic for 1000[m] from a given initial position with $\tplan = 3$[sec].  
Each highway scenario contains 3 static obstacles and a number of moving vehicles as dynamic obstacles, where the number of moving vehicles in each scenario is randomly selected between 5 and 25 vehicles at the beginning of each scenario. 
The initialization of each dynamic obstacle and its corresponding probability density function $\pdf$ with each $j\in\J$ are performed in the same way as explained in Section \ref{subsec: single_plan_sim}.
Each scenario is simulated for 10 trials resulting in a total of 10,000 simulation cases.
\Ram{explain what you mean by a trial here.}
In each scenario, the ego vehicle is initialized in the center of a random lane and the initial speed of the ego vehicle is randomly selected from between 15[m/s] to 25[m/s].

Each moving vehicle is set to maintain its speed and start within 120[m] ahead of the ego vehicle's initial position, so that the ego vehicle could encounter dense traffic immediately from the beginning.
Table \ref{table: multiplan highway result} presents \riskmethodname{}, CCPBA, Cantelli MPC, and REFINE's results for all 10,000 cases of the 3 lane multiple planning horizon experiment.
In this experiment, a success is defined as being able to successfully navigate through the entire 1000m highway and reach the goal.
\Ram{the rest of this paragraph is just repeating what appears in the table. Maybe instead of just writing out something that a reader can look at it would be helpful to compare performance in some way?}
\riskmethodname{} was able to successfully navigate through the entire stretch of highway 74.8\% of the time, came to a safe stop partially through the highway 24.4\% of the time and crashed 0.8\% of the time.
CCPBA was able to successfully through the entire stretch of highway 19.4\% of the time, came to a safe stop 79.6\% of the time and crashed 1\% of the time.
Cantelli MPC was only able to successfully through the entire stretch of highway 17.5\% of the time, and crashed 82.5\% of the time, and never came to a safe stop due to the lack of a braking maneuver.
% Compared to the single planning iteration experiments, \riskmethodname{} had a small drop in success rate. 
% This was expected as over the full highway scenario, once \riskmethodname{} has executed an action, it may start the next planning iteration from an initial condition where it is difficult to find a solution that satisfies the constraint, while getting close to the specified waypoint.
% This was also the case for CCPBA and Cantelli MPC.
% This was also the case for CCPBA, however with CCPBA, due to the fact that it chose not to execute the lane change maneuver more often in earlier parts of each trial, it often found itself in scenarios where it would be stuck behind and beside other vehicles. 
% Whereas if it had been more aggressive and executed the lane change earlier when it had a chance. that it could have avoided these situations.
% \challen{Above I'm describing scenarios where you have a tight window to overtake another car, and if you miss the window, then you get stuck in slower traffic. If you have a clearer way to explain this feel free to change it}


\begin{table}[!tb]
    \centering
    \begin{tabular}{|c||c|c|c|c|}
    \hline 

    \multirow{2}{*}{\textbf{Method}} & \textbf{Success} & \textbf{Crash} & \textbf{Safely} & \textbf{Mean} \\
    & \textbf{[\%]} & \textbf{[\%]} & \textbf{Stop [\%]}  & \textbf{Solve Time}\\\hline
    \riskmethodname{} & \textbf{74.8} & 0.80 & 24.4 & 0.412 $\pm$ 0.271 \\\hline
    CCPBA & 42.5 & 0.4 & 57.1 & \textbf{0.291 $\pm$ 0.124}  \\ \hline
    Cantelli MPC & 23.5 & 76.5 & \textbf{0.00} & 0.643 $\pm$ 0.141 \\\hline
    REFINE & 61.0 & \textbf{0.00} & 39.0 & 0.341 $\pm$ 0.113  \\\hline
    
    % \methodname & 27\% & 0\% & 73\% & 16.5927[m/s] &  (0.2537[s], 1.3042[s])  \\ \hline
    \end{tabular}
    \caption{Simulation results comparing \riskmethodname{} to CCPBA, Cantelli MPC and REFINE on a 1000m stretch of dense highway. 
    A successful trial means the ego vehicle was able to successfully reach the 1000m goal without crashing or coming to a stop.}
    
    \label{table: multiplan highway result}
\end{table}

% Table \ref{table: multiplan highway result} provides the statistic of simulation results using the three methods.
% Unsurprisingly the ego vehicle with \riskmethodname{} being applied crashes in some simulation scenario, because \riskmethodname{} only ensures the vehicle safety with confidence level $1-\epsilon$.
% However, with the guarantee of vehicle safety being sacrificed, the ego vehicle is able to travel faster and more aggressively under the \riskmethodname{} planning framework, thus still achieves the highest successful rate among the three testing methods. 

\subsubsection{Left Turning}
 The aim of this experiment is to evaluate how different risk thresholds ($\epsilon$) affect the behavior and performance of \riskmethodname{} over a single planning iteration.
 Unprotected left turns are ideal scenarios to evaluate this over a single planning iteration.
 In these scenarios being less conservative has a large effect on the ability of the ego vehicle to complete the left turn faster by navigating through tight windows in the traffic of oncoming vehicles.
 This experiment sets the risk threshold to 0.01, 0.05, 0.10 and 0.20 and has the ego vehicle navigate through a 1000 randomly generated unprotected left turning scenarios. 
 In each scenario, the ego vehicle is tasked with executing an unprotected left turn across two oncoming lanes at a 4-way intersection as depicted in Figure \ref{fig: left_turn}.
 Each scenario contains between 4 to 6 static obstacles occupying the horizontal lanes of the intersection and up to 4 dynamic obstacles that drive through the intersection in the vertical lanes, where the number of static and dynamic obstacles are randomly selected each scenario.
 The starting lanes and initial positions of the dynamic obstacles are also randomly selected each scenario.
 The initial speeds of the dynamic obstacles are randomly sampled from between 12[m/s] and 17[m/s].
\Ram{what is the pdf of the obstacles?}
 
 Table \ref{table: left-turning} summarizes the results of the left turning experiment.
 As the risk threshold $\epsilon$ is increased, we see a reduction in the Average Time To Goal (ATTG) and Maximum Time To Goal (MTTG) as the ego vehicle is less conservative with higher $\epsilon$'s and thus executes the unprotected left turns more quickly.
 \Ram{maybe its worth rerunning these experiments with an even larger epsilon?}
 % At $\epsilon$ = 1\%, \riskmethodname{} is able to complete 99.6\% of the turns without a crash, however, it has a relatively large ATTG of 12.6s since it waits for nearly all the obstacle vehicles to go through the intersection before executing the left turn.
 % At $\epsilon$ = 5\%, \riskmethodname{} is able to navigate through 99.0\% of the turns without a crash, with a ATTG of 9.2s. It crashed 1.0\% of the time.
 % At $\epsilon$ = 10\%, \riskmethodname{} is only able to complete 97.9 without crashing. 
 % However, due to its reduced conservatism it has a the lowest ATTG and is able to take more risky turns and navigate through the turn when it only has a small window to do so.
 % This reduced conservatism results in crashes 2.1\% of the time.


 \begin{figure}[!tb]
    \centering
    \includegraphics[trim={0cm, 7.cm, 10.cm, 0.2cm},clip,width=1\columnwidth]{figures/left_turn.pdf}
    \caption{Example of a simulated unguarded left turning trial where the ego vehicle (black) navigates through a gap in the oncoming traffic to successful execute the unguarded left turn.
    Forward reachable sets are shown in green.
    Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
    Probability distributions are illustrated as purple and blue ellipses where the probability density from low to high is illustrated from blue to purple.
    }
    \label{fig: left_turn}
\end{figure}
 
\begin{table}[!tb]
    \centering
    \begin{tabular}{|c||c|c|c|c|}
    \hline 

    \textbf{$\epsilon$} & \textbf{Success [\%]} & \textbf{Crash[\%]} & \textbf{ATTG [s]} & \textbf{MTTG [s]} \\ \hline
    0.01 & 100 & 0.00 & 9.55 & 14.7 \\\hline
    0.05 & 100 & 0.00 & 8.38 & 13.8\\ \hline
    0.10 & 100 & 0.00 & 6.51 & 13.6  \\\hline
    0.20 & 100 & 0.00 & \textbf{6.26} & \textbf{11.3} \\\hline
    
    % \methodname & 27\% & 0\% & 73\% & 16.5927[m/s] &  (0.2537[s], 1.3042[s])  \\ \hline
    \end{tabular}
    \caption{Simulation results over a single planning iteration for \riskmethodname{} executing a left turn at different risk thresholds.
    Average Time To Goal (ATTG) and Maximum Time To Goal (MTTG) are only taken over successful trials.}
    
    \label{table: left-turning}
\end{table}

\subsubsection{Ablation Study}
\label{subsubsec: planning time without relaxation}
% \jinsun{@Challen, we need an experiment to show that planning with the original chance constraint in \opt{} with monte carlo sucks because it's too slow}

This section performs an ablation study to evaluate the effectiveness of each component of \riskmethodname{} (see Table \ref{table: ablation study}).
In this ablation study, we examine the performance of 3 algorithms, each of which has a certain aspect of \riskmethodname{} removed.
Namely, the 3 algorithms are: \riskmethodname{} (No Analytical Gradient), Monte-Carlo RTD (Discrete) and Monte-Carlo RTD (Continuous).
% Monte-Carlo RTD (Discrete + Relaxation), Monte-Carlo RTD (continuous + relaxation).
% identify the components that make \riskmethodname{} so successful.
For \riskmethodname{} (No Analytical Gradient), we examine the performance of \riskmethodname{} without providing the constraint gradient described in Section \ref{subsec:gradient}. 
Instead we allow IPOPT to compute a numerical gradient during the optimization.
In the other 2 algorithms, instead of leveraging our over-approximation to the risk of collision from Section \ref{sec: chance constraint}, we instead replace this with a Monte Carlo style sampling method to estimate the risk of collision.
For Monte-Carlo RTD (Discrete), to find a viable control parameter, we sample discrete points from the control parameter space $\P$ in a similar fashion to \cite{manzinger2020using}
Additionally, we sample trajectories for each obstacle and count the trajectories that intersect with the ego vehicle trajectory parameterized by the sampled control parameter $p \in \P$ to estimate the risk of collision in this method.
% $\E\big(t,z_0,p\big)$ at a time $t$ such that $t$ is set to be the time at midpoint of the interval $T_j$ to approximate the left hand side of the chance constraint provided in \eqref{eq: chance constraint def}. 
% at the $j$-th time interval that corresponds to  lie inside the zonotope $\xi_j(z_0,p)\oplus\zonocg{0}{\Gobs}$ to approximate the left hand side of the chance constraint provided in \eqref{eq: chance constraint def}. 

% For Monte-Carlo RTD (Discrete + Relaxation) ((MCRTD(D+R)), we sample control parameters in the same way as Monte-Carlo RTD (Discrete), however in this algorithm we estimate the risk of collision by sampling from $\pdf(\cdot\mid i,j)$ and determining in the number of samples in each right triangle $\T\in\bT_{j}(z_0)$. 
% We then sum up all the probability mass in all the right triangles and zonotopes corresponding to the sampled control parameter $p$ to estimate the relaxed chance constraint in \optE{}, hence the name Monte-Carlo RTD (Discrete + Relaxation).
Monte-Carlo RTD (Continuous) estimates the risk of collision in the same way as Monte-Carlo RTD (Discrete), however in this algorithm we assume the control parameter space $\P$ is continuous and allow IPOPT to compute a numerical gradient and search $\P$ for a control parameter $p$ that satisfies the \eqref{eq: chance constraint def} as estimated with the Monte-Carlo method.
% Monte-Carlo RTD (Continuous + Relaxation) ((MCRTD(C+R)) estimates the risk of collision in the same way as Monte-Carlo RTD (Discrete + Relaxation) and determines which control parameter to use in the same way as Monte-Carlo RTD (Continuous).

The results of the ablation study can be found in Table \ref{table: ablation study}.
From the ablation study it is evident that replacing the closed-form over-approximation with Monte-Carlo sampling methods causes a large increase in the time needed to estimate the risk of collision and generate a motion plan.
Monte-Carlo RTD (Discrete) and Monte-Carlo RTD (Continuous) achieve similar success rates to \riskmethodname{}, but had average solve times of 38.2s and 45.0s, respectively.
Both of these times are too slow to be able to achieve real-time performance.
We note that reducing the number of samples they use to estimate the risk of collision would reduce this solve time, but will have a detrimental effect on the success rate of methods as they may greatly under-approximate the true risk of collision with low sample numbers.
Without the analytical gradients being provided, \riskmethodname{} is still unable to achieve real-time planning and requires an average time of 7.81s to generate a motion plan, which is too slow to operate in real-time.
It is evident from these results that both the analytical gradient and the closed form over-approximation play important roles in being able to generate motions plans in real-time.
% that give while giving a reliable estimation the risk of collision and achieving a good success rate.




\begin{table}[!tb]
    \centering
    \begin{tabular}{|c||c|c|c|c|}
    \hline 

     \multirow{2}{*}{\textbf{Algorithm}} &  \multirow{2}{*}{\textbf{Success [\%]}} &  \multirow{2}{*}{\textbf{Crash[\%]}} & \textbf{Other} & \textbf{Solve} \\
      &  &  & \textbf{Action[\%]} & \textbf{time [s]} \\ \hline
    \color{blue}\riskmethodname{}(NAG) & 73.9 & 1.1 & 25.0 & 7.81 \\\hline
    MCRTD(D) & 85.0 & 3.2 & \textbf{11.8} & 38.2 \\ \hline
    % MCRTD(D+R) & 81.0 & 1.9 & 17.1 & 6.20  \\\hline
    \color{blue} MCRTD(C) & \textbf{85.2} & 2.1 & 12.7 & 45.0  \\\hline
    % MCRTD(C+R) & 82.1 & 1.2 & 16.7 & 8.30  \\\hline
    \color{blue} \riskmethodname{} & 81.8 & \textbf{0.0} & 18.2 & \textbf{0.41}  \\\hline
    
    % \methodname & 27\% & 0\% & 73\% & 16.5927[m/s] &  (0.2537[s], 1.3042[s])  \\ \hline
    \end{tabular}
    \caption{Single planning iteration results using the \riskmethodname{} variants considered in the ablation study.
    ``Other Action" encompasses the trials where each method did not complete the lane change maneuver, but instead either executed a safe stop maneuver or decided to keep driving in lane. \riskmethodname{} (No Analytical Gradient) is abbreviated as \riskmethodname{} (NAG), Monte-Carlo RTD (Discrete) is abbreviated as MCRTD(D) and Monte-Carlo RTD (Continuous) is abbreviated as MCRTD(C).
    }
    
    \label{table: ablation study}
\end{table}


\subsection{Hardware}





% \clearpage
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.325\textwidth}
%          \includegraphics[trim={1cm, 7.8cm, 9cm, 0cm},clip,width=\textwidth]{figures/merge_risk.pdf}
%          \caption{\riskmethodname{} utilized.}
%          \label{fig: simulation result 1-riskrtd}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.325\textwidth}
%          \includegraphics[trim={1cm, 7.8cm, 9cm, 0cm},clip,width=\textwidth]{figures/merge_ccpba.pdf}
%          \caption{CCPBA utilized.}
%          \label{fig: simulation result 1-CCPBA}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.325\textwidth}
%          \includegraphics[trim={1cm, 7.8cm, 9cm, 0cm},clip,width=\textwidth]{figures/merge_cantelli.pdf}
%          \caption{Cantelli MPC utilized.}
%          \label{fig: simulation result 1-cantelli}
%      \end{subfigure}
%     \caption{Example of a simulated scenario in which \riskmethodname{} and CCPBA are able to navigate the ego vehicle (black) to the provided waypoint (black cross) through a lane change maneuver solved by one planning iteration, while Cantelli MPC results in a crash.
%     Forward reachable sets are shown in green.
%     Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
%     Probability distributions are illustrated as colored ellipses where the probability density from low to high are illustrated from blue to yellow.
%     Note that for visualization purposes we have buffered the probability distributions shown in this figure by the footprints of the obstacles}
%     \label{fig: single planning iteration}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.325\textwidth}
%          \includegraphics[trim={1cm, 7.8cm, 14.5cm, 0cm},clip,width=\textwidth]{figures/merge_risk.pdf}
%          \caption{\riskmethodname{} utilized.}
%          \label{fig: simulation result 1-riskrtd}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.325\textwidth}
%          \includegraphics[trim={1cm, 7.8cm, 14.5cm, 0cm},clip,width=\textwidth]{figures/merge_ccpba.pdf}
%          \caption{CCPBA utilized.}
%          \label{fig: simulation result 1-CCPBA}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.325\textwidth}
%          \includegraphics[trim={1cm, 7.8cm, 14.5cm, 0cm},clip,width=\textwidth]{figures/merge_cantelli.pdf}
%          \caption{Cantelli MPC utilized.}
%          \label{fig: simulation result 1-cantelli}
%      \end{subfigure}
%     \caption{Example of a simulated scenario in which \riskmethodname{} and CCPBA are able to navigate the ego vehicle (black) to the provided waypoint (black cross) through a lane change maneuver solved by one planning iteration, while Cantelli MPC results in a crash.
%     Forward reachable sets are shown in green.
%     Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
%     Probability distributions are illustrated as colored ellipses where the probability density from low to high are illustrated from blue to yellow.
%     Note that for visualization purposes we have buffered the probability distributions shown in this figure by the footprints of the obstacles}
%     \label{fig: single planning iteration}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.332\textwidth}
%          \includegraphics[trim={0cm, 7.4cm, 15.5cm, 0cm},clip,width=\textwidth]{figures/merge_risk_v2.pdf}
%          \caption{\riskmethodname{} utilized.}
%          \label{fig: simulation result 1-riskrtd}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.322\textwidth}
%          \includegraphics[trim={0cm, 7.4cm, 16.1cm, 0cm},clip,width=\textwidth]{figures/merge_ccpba_v2.pdf}
%          \caption{CCPBA utilized.}
%          \label{fig: simulation result 1-CCPBA}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.322\textwidth}
%          \includegraphics[trim={0cm, 7.4cm, 16.1cm, 0cm},clip,width=\textwidth]{figures/merge_cantelli_v2.pdf}
%          \caption{Cantelli MPC utilized.}
%          \label{fig: simulation result 1-cantelli}
%      \end{subfigure}
%     \caption{Example of a simulated scenario in which \riskmethodname{} and CCPBA are able to navigate the ego vehicle (black) to the provided waypoint (black cross) through a lane change maneuver solved by one planning iteration, while Cantelli MPC results in a crash.
%     Forward reachable sets are shown in green.
%     Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
%     Probability distributions are illustrated as colored ellipses where the probability density from low to high are illustrated from blue to yellow.
%     Note that for visualization purposes we have buffered the probability distributions shown in this figure by the footprints of the obstacles}
%     \label{fig: single planning iteration}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.332\textwidth}
%          \includegraphics[trim={0cm, 7.4cm, 15.5cm, 0cm},clip,width=\textwidth]{figures/merge_risk_v3.pdf}
%          \caption{\riskmethodname{} utilized.}
%          \label{fig: simulation result 1-riskrtd}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.322\textwidth}
%          \includegraphics[trim={0cm, 7.4cm, 16.1cm, 0cm},clip,width=\textwidth]{figures/merge_ccpba_v3.pdf}
%          \caption{CCPBA utilized.}
%          \label{fig: simulation result 1-CCPBA}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.322\textwidth}
%          \includegraphics[trim={0cm, 7.4cm, 16.1cm, 0cm},clip,width=\textwidth]{figures/merge_cantelli_v3.pdf}
%          \caption{Cantelli MPC utilized.}
%          \label{fig: simulation result 1-cantelli}
%      \end{subfigure}
%     \caption{Example of a simulated scenario in which \riskmethodname{} and CCPBA are able to navigate the ego vehicle (black) to the provided waypoint (black cross) through a lane change maneuver solved by one planning iteration, while Cantelli MPC results in a crash.
%     Forward reachable sets are shown in green.
%     Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
%     Probability distributions are illustrated as colored ellipses where the probability density from low to high are illustrated from blue to yellow.
%     Note that for visualization purposes we have buffered the probability distributions shown in this figure by the footprints of the obstacles}
%     \label{fig: single planning iteration}
% \end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}
%          \includegraphics[trim={0cm, 9.15cm, 8.4cm, 0cm},clip,width=\textwidth]{figures/merge_risk_v4.pdf}
%          \caption{\riskmethodname{} utilized.}
%          \label{fig: simulation result 1-riskrtd}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.49\textwidth}
%          \includegraphics[trim={0cm, 9.15cm, 8.4cm, 0cm},clip,width=\textwidth]{figures/merge_ccpba_v4.pdf}
%          \caption{CCPBA utilized.}
%          \label{fig: simulation result 1-CCPBA}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.49\textwidth}
%          \includegraphics[trim={0cm, 9.15cm, 8.4cm, 0cm},clip,width=\textwidth]{figures/merge_cantelli_v4.pdf}
%          \caption{Cantelli MPC utilized.}
%          \label{fig: simulation result 1-cantelli}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\textwidth}
%          \includegraphics[trim={0cm, 9.15cm, 8.4cm, 0cm},clip,width=\textwidth]{figures/merge_refine_v4.pdf}
%          \caption{REFINE utilized.}
%          \label{fig: simulation result 1-refine}
%      \end{subfigure}
%     \caption{Example of a simulated scenario in which \riskmethodname{} and CCPBA are able to navigate the ego vehicle (black) to the provided waypoint (black cross) through a lane change maneuver solved by one planning iteration, while Cantelli MPC results in a crash.
%     Forward reachable sets are shown in green.
%     Obstacles are shown in white and are marked by their indices to make them trackable among different time instances.
%     Probability distributions are illustrated as colored ellipses where the probability density from low to high are illustrated from blue to yellow.
%     Note that for visualization purposes we have buffered the probability distributions shown in this figure by the footprints of the obstacles}
%     \label{fig: single planning iteration}
% \end{figure*}

==> sections_long/08_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

% This work proposes ARMTD as a real-time, receding-horizon manipulator trajectory planner with safety guarantees.
% The method proposes novel reachable sets for arms, which enable safety.
% ARMTD can enforce safety on top of an unsafe path planner such as RRT*, shown in both simulation and on hardware.
% % Furthermore, ARMTD is able to outperform the existing CHOMP planner in terms of task completion and safety, while not requiring much more planning time.
% Of course, ARMTD has limitations: it may not perform in real time without parallelization, is only demonstrated on 6-DOF planning problems, and has not yet been demonstrated planning around humans.
% However, because ARMTD uses time-varying reachable sets, it can readily extend to dynamic environments, uncertainty such as tracking error, and planning with grasped objects.
% The results in this work show promise for practical, safe robotic arm trajectory planning.

% \pat{I think we need quite a bit more here... I really don't think the utility of ARMTD comes through unless we talk about dynamic obstacles/obstacles w bounded velocity and how those fit naturally into this framework, as well as potentially how to deal with the tracking error/manipulator dynamics, and how to add the grasped object volume onto the FRSs... yeah I just feel like we need to sell it a bit more.}

